Learning Navigation Costs from Demonstration in Partially Observable Environments

This paper focuses on inverse reinforcement learning (IRL) to enable safe and efficient autonomous navigation in unknown partially observable environments. The objective is to infer a cost function that explains expert-demonstrated navigation behavior while relying only on the observations and state-control trajectory used by the expert. We develop a cost function representation composed of two parts: a probabilistic occupancy encoder, with recurrent dependence on the observation sequence, and a cost encoder, defined over the occupancy features. The representation parameters are optimized by differentiating the error between demonstrated controls and a control policy computed from the cost encoder. Such differentiation is typically computed by dynamic programming through the value function over the whole state space. We observe that this is inefficient in large partially observable environments because most states are unexplored. Instead, we rely on a closed-form subgradient of the cost-to-go obtained only over a subset of promising states via an efficient motion-planning algorithm such as A* or RRT. Our experiments show that our model exceeds the accuracy of baseline IRL algorithms in robot navigation tasks, while substantially improving the efficiency of training and test-time inference.

==> tex/Approach.tex <==
\section{Technical Approach}
\label{sec:technical_approach}
Our approach to Problems~\ref{pb:1} and ~\ref{pb:2} is to encode a cost learning model and a planning model in a fully differentiable computation graph, and learn the parameters $\theta$ in a gradient-based approach as shown in Figure~\ref{fig:approach}. First, we represent $\hat{c}_t^\theta$ as a neural network with inputs $x \in \mathcal{X}$, $u\in\mathcal{U}$, and $z_{1:t} \in \mathcal{Z}^t$ and parameters $\theta$. Second, we propose an efficient differentiable planning model that returns a stochastic policy $\pi_t^{\theta}$ given a fixed estimated cost $\hat{c}_t^{\theta}$ while requiring that $\pi_t^{\theta}$ is differentiable with respect to $\theta$. Third, we optimize the performance loss $\mathcal{L}(\theta)$ of the inferred policy $\pi_t^{\theta}$ with the expert demonstrations $\mathcal{D}$ using gradient descent over the parameters $\theta$.


\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/CostNeuralNet}
  \caption{Neural net representation of the cost function. The RNN, parameterized by $\theta_1$, takes in the observations $z_{1:t}$ sequentially and outputs a low-dimensional latent map representation $\hat{m}_t$. The CNN, parameterized by $\theta_2$, estimates the cost function $\hat{c}_t^{\theta}$ from the latent map, state and control. The learnable parameters are $\theta = \crl{\theta_1, \theta_2}$.}
  \label{fig:cost_neural_net}
\end{figure}
%We consider the problem of learning a parameterized mapping $g(\cdot|\theta):\mathcal{Z} \rightarrow \hat{C}$ (from observations to cost functions) so that $\pi(\cdot | \hat{c})$ (policy on the learned cost function) obtains a low cost with respect to the true cost function $c$. Our general approach, shown in Fig~\ref{fig:approach1} can be described as taking the gradient of the loss function with respect to the parameters $\theta$, where the loss function can be defined on the true cost $c^{*}$ or on some expert policy $\pi^*$. In order to perform gradient descent on the loss function, we have to ensure that the gradient can be backpropagated through the planning algorithm. Specifically, we have to ensure $\frac{\partial J}{\partial \pi}$, $\frac{\partial \pi}{\partial \hat{c}}$, and $\frac{\partial \hat{c}}{\partial \theta}$ exist and are correctly computed in backpropagation. 



\subsection{Cost Function Representations}
\label{subsec:cost_repr}
Learning a cost function from observations can be encoded as a neural net in general as shown in Figure~\ref{fig:cost_neural_net}. We first train a recurrent neural net (RNN) with parameters $\theta_1$ that consumes the high-dimensional observations sequentially and outputs a low-dimensional latent environment representation $\hat{m}_t$. The RNN models the dependence of the sequential observations on the underlying state of the environment. The idea of extracting occupancy information from observations and keeping track of an internal latent map representation is also explored in ~\cite{Gupta_CMP17, Oh_ActPred15}. \TW{~\cite{Khan_MACN_ICLR18} does not have this RNN strucuture. It processes the observations as in VIN (the CONV block in Fig. 3). The controller is LSTM though.} The latent map representation $\hat{m}_t$ is fed into a convolutional neural net (CNN) with parameters $\theta_2$, along with state $x$ and control $u$. It encodes spatial feature from the latent map to produce a cost function $\hat{c}_t^{\theta}$ for planning. With the implementation of neural nets as cost function representation, we emphasize that the output cost function $\hat{c}_t^{\theta}$ is differentiable with respect to the network parameters $\theta = \{\theta_1, \theta_2\}$. We will later learn the parameters $\theta$ as part of the policy learning process. 

\label{subsubsec:occ_cost}
\begin{figure}[ht]
\centering
\begin{subfigure}[b]{.5\linewidth}
  \centering
  \includegraphics[width=\linewidth]{fig/map.png}
  \caption{2D grid map}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}[b]{.5\linewidth}
  \centering
  \includegraphics[width=\linewidth]{fig/obs.png}
  \caption{Robot observation}
  \label{fig:sub2}
\end{subfigure}
\caption{An example of a robot, indicated in blue, attempting to navigate to the goal, indicated in red, in a 2D grid cell environment. The map has size $16\times16$ where black regions are obstacles and white regions are free space. The robot observable region is a $5\times5$ box around its current state and the grey regions are not observed.}
 \label{fig:map_and_obs}
\end{figure}
\subsubsection{Occupancy-based Cost Function Representation} \TW{I think this is a subsection of the general cost function representation above but there is no subsubsection 4.1.2 as you mentioned last time}
As a specific instantiation of the general problem setting stated above, we choose to demonstrate the idea of learning cost functions through differentiable planning model by considering navigation tasks in a 2D grid cells. Let $m^* \in \{0, 1\}^n$ be a true occupancy map, so $m^*[x] = \{0,1\}$ is the occupancy label at state $x$. The robot receives binary observations $z_t = H(x_t) m^*$, where $z_t \in \{0, 1\}^n$ and the diagonal matrix $H(x_t) \in \{0,1\}^{n \times n}$ consists of ones for observable states and zeros for unobservable states, capturing the local field of view of the robot at $x_t$. An example of such occupancy map and robot observation is shown in Figure~\ref{fig:map_and_obs}. \\ \\
Next, we show a specific occupancy-based design of the cost function representation for navigation in 2D grid environments. Instead of using a standard RNN model, we accumulate the log-odds ratio of the occupancy probability of each cell. Let $\hat{m} \in \{0, 1\}^n$ be the map occupancy estimate which is a collection of $n$ independent Bernoulli random variables. The probability density of $\hat{m}$ can be updated via an observation model which is a sigmoid function parameterized by $\theta_1$, indicating how much we trust the observation measurements,
\begin{equation}
\begin{aligned}
p(z_t|\hat{m};\theta_1) &:= 
\begin{cases}
    \sigma(\theta_1),& \text{if } z_t = \hat{m}\\
    \sigma(-\theta_1), & \text{if } z_t \neq \hat{m}
\end{cases} \\
&= \sigma((2z_t-1)(2\hat{m}-1)\theta_1) \;.
\end{aligned}
\end{equation}
Note that we drop the argument $x$ for brevity since the random variables $\hat{m}[x]$ are independent. We choose the sigmoid observation model demonstrate the feasibility of the model in the 2D grid environment and it can be replace by a CNN if the observations are more complicated. We can simplify the log-odds ratio of the observation model as
\begin{equation}
\ln \frac{p(z_t|\hat{m}=1)}{p(z_t|\hat{m}=0)} = (2z_t-1)\theta_1 \;.
\end{equation}
Given a history of observations $z_{1:t}$, the robot estimates the log-odds ratio $\lambda \in \mathbb{R}^n$ of the occupancy probability, which can be decomposed using Bayes rule as a sum of the log-odds ratio of the observation model over time,
\begin{equation}
\begin{aligned}
\lambda(\hat{m} \mid z_{1:t}) &:= \ln \frac{p(\hat{m}=1 \mid z_{1:t})}{p(\hat{m}=0 \mid z_{1:t})} \; \\
&= \lambda(\hat{m}) + \sum_{\tau=1}^t (2z_{\tau}-1)\theta_1
\end{aligned}
\end{equation}
with some prior $\lambda(\hat{m})$. The log-odds ratio $\lambda(\hat{m} \mid z_{1:t})$ can be regarded as the hidden state $h_t$ in Figure~\ref{fig:cost_neural_net} and accumulates $(2z_t-1)\theta_1$ for each new observation $z_t$. Finally, the output is the probability density function of the map estimate $\hat{m}$, which can be recovered from the log-odds $\lambda(\hat{m} \mid z_{1:t})$ by 
\begin{equation}
\begin{aligned}
p_t^{\theta_1}(\hat{m}) &:= p(\hat{m} = 0 \mid z_{1:t}) \\
              &= \frac{1}{1+\exp(\lambda(\hat{m} \mid z_{1:t}) )} \;.
\end{aligned}
\end{equation}
We would like to emphasize that $p_t^{\theta_1}(\hat{m})$ is a function of $\theta_1$ through $\lambda(\hat{m} \mid z_{1:t})$ as we require that the output is differentiable with respect to $\theta_1$. \\ \\
Instead of implementing a CNN block in Figure~\ref{fig:cost_neural_net}, we adopt an induced cost function from map estimate. Implementing a CNN is not necessary as we explicitly model the occupancy probability of each cell in the 2D environment while in the general case we do not know what the hidden state $h_t$ represents. The cost function can be induced from the map estimate $\hat{m}$ as follows. Let the actual cost of each control be
\begin{equation}
c(x_t,u_t):=
    \begin{cases}
    s, \; & \text{if} \: \hat{m}[x_t] = 0 \text{ and } \hat{m}[f(x_t, u_t)] = 0\\
    l, & \text{if } \hat{m}[x_t] = 1 \text{ or } \hat{m}[f(x_t, u_t)] = 1 
    \end{cases}
\end{equation}
where $s$ and $l$ are some small and large positive constants (for example, $s=\lVert x_t-f(x_t, u_t) \rVert_2 $ and $l = 100s$\TW{This looks too arbitrary. Also $x_t$ is not the coordinate of the grid}). The estimated cost function $\hat{c}^{\theta}_t$ is the expected value of $c$,
\begin{equation}
\begin{aligned}
\label{eq:chat}
\hat{c}_t^{\theta}(x_t, u_t) &= \mathbb{E}_{\hat{m}} [c(x_t, u_t)] \\
&= p_t^{\theta_1}(\hat{m}[x_t])p_t^{\theta_1}(\hat{m}[f(x_t, u_t)]) \times s + \\
                          &\Big(1-p_t^{\theta_1}(\hat{m}[x_t])p_t^{\theta_1}(\hat{m}[f(x_t, u_t)])\Big) \times l \; .
\end{aligned}
\end{equation}
Note that the output $\hat{c}_t^{\theta}(x_t, u_t)$ is differentiable with respect to $\theta_1$ through $p_t^{\theta_1}(\hat{m})$. \\ \\
In summary, we design a cost function representation which is differentiable with respect to its parameters in 2D grid environments. The cost function is induced from the occupancy probability of the cells which is updated by the log-odds ratio of the parameterized observation likelihood. 

\subsection{Differentiable planning model}
\label{subsec:diff_plan}
In this section, we will develop planning algorithms over the learned cost function $\hat{c}_t^{\theta}$ while ensuring that the output stochastic policy $\pi_t^{\theta}$ is differentiable with respect to $\hat{c}_t^{\theta}$. Value iteration networks (VIN)~\cite{Tamar_VIN16} has shown that the value iteration algorithm can be approximated by a neural net architecture with convolutional and maxpooling layers. While VIN makes the planning model differentiable and allows backpropagation, we argue that convolutional operations over the entire state space are computationally expensive and do not scale with the size of the state space and the planning horizon. As a solution to this issue, we first propose a differentiable dynamic programming model, inspired by VIN, that solves the deterministic shortest path problem on $\hat{c}_t^{\theta}$. We then propose a differentiable A* algorithm that only performs local convolutional operations that encode Bellman backups on a subset of promising states.

\subsubsection{Differentiable dynamic programming algorithm}
\label{subsubsec:diff_dp}
The original VI module in VIN solves the infinite horizon stochastic shortest path problem. Inspired by the VI module, we propose a differentiable dynamic programming (DP) algorithm that solves the finite-horizon deterministic shortest path problem as follows. Let $V(x)$ be the optimal cost-to-go from each state $x$ to $x_g$, with respect to the cost function $\hat{c}_t^{\theta}$,
\begin{equation}
\begin{aligned}
& V(x) =  \min_{u_{1:T-1}}  \sum_{\tau=1}^{T-1} \hat{c}_t^{\theta}(x_{\tau}, u_{\tau}) \\
& \text{s.t.}\;\; x_{\tau+1} = f(x_{\tau}, u_{\tau}),\; x_1 = x,\; x_T = x_g.
\end{aligned}
\end{equation}
The optimal cost-to-go $V(x)$ for all states $x$ can be obtained at the last step of the differentiable DP algorithm (Algorithm~\ref{alg:1}). To enforce differentiability, we implement the Bellman equations in line 10 and 11 of Algorithm~\ref{alg:1} with neural net layers as inspired by VIN. We implement $V(x)$ as a vector of size $|\mathcal{X}|$ and $Q(x,u)$ as a matrix of size $|\mathcal{X}|\times|\mathcal{U}|$. Let $\delta(x) \in \crl{0,1}^{|\mathcal{X}|}$ be a kronecker delta function
\begin{equation}
\begin{aligned}
    \delta(x) = 
    \begin{cases}
    1, \text{ if } x = 0, \\
    0, \text{ otherwise.}
    \end{cases}
\end{aligned}
\end{equation}
The optimal cost-to-go at the next state $V(f(x_{\tau}, u_{\tau}))$ can be obtained by having a convolutional layer on $V(x)$ with $\delta(f(x_{\tau}, u_{\tau})-x)$ as the convolutional kernel that accounts for the deterministic transitions from $x_{\tau}$ to $f(x_{\tau}, u_{\tau})$,
\begin{equation}
\begin{aligned}
V(f(x_{\tau}, u_{\tau})) &= \sum_{s=0}^{|\mathcal{X}-1|} \delta(f(x_{\tau}, u_{\tau})-s) V(s) 
\end{aligned}
\end{equation}
 The quantity $Q(x_{\tau}, u_{\tau})$ is then min-pooled along the control channel to get $V(x_{\tau})$ for the next iteration. \TW{This does not look like the algorithmic environment and I cannot use the Return command in function.}
\begin{algorithm}[ht]
\caption{Differentiable Dynamic Programming Algorithm}
\label{alg:1}
\begin{algorithmic}[1]
\STATE {\bfseries Input:} Current state $x_t$, goal state $x_g$, cost function $\hat{c}_t^{\theta}$, deterministic transition $f$
\FUNCTION{Conv($V(x), \delta({f(x_{\tau},u_{\tau})} - x) $)}
    \STATE {\bfseries return} $\sum_{s=0}^{|\mathcal{X}-1|} \delta(f(x_{\tau}, u_{\tau})-s) V(s) $
\ENDFUNCTION

\FUNCTION{Minpool($Q(x_{\tau},u_{\tau})$)}
    \STATE {\bfseries return} $\min_{u_{\tau} \in \mathcal{U}} \crl{Q(x_{\tau}, u_{\tau})}$
\ENDFUNCTION

\STATE $V(x_g) \leftarrow 0$, $V(x) \leftarrow \infty \; \forall x \in \mathcal{X} \setminus x_g$

\FOR{$\tau = T-1:1$}
    \STATE $Q(x_{\tau}, u_{\tau}) \leftarrow \hat{c}_t^{\theta}(x_{\tau}, u_{\tau}) + \text{Conv}(V(x), \delta({f(x_{\tau},u_{\tau})} - x)), \; \forall x_{\tau} \in \mathcal{X} \setminus x_g$ and  $\forall u_{\tau} \in \mathcal{U}$
    \STATE $V(x_{\tau}) \leftarrow \text{Minpool }( Q(x_{\tau}, u_{\tau})), \; \forall x_{\tau} \in \mathcal{X} \setminus x_g$ 
\ENDFOR
\STATE {\bfseries Output:} Policy $\pi_t^{\theta}(u_t|x_t) = \frac{\exp{\big(-Q(x_t, u_t)\big)}}{\sum_{u_t'\in \mathcal{U}}\exp{\big(-Q(x_t, u_t')\big)}}$ 
\end{algorithmic}
\end{algorithm}
\\ \\
The differentiable DP algorithm is a straightforward extension of the VI module in VIN with deterministic transitions and finite planning horizon by having kronecker delta convolutional kernels and clamping $V(x_g) = 0 $ throughout the iterations. Both the VI module and the differentiable DP algorithm output differentiable policy by using neural net layers and require convolutional operation over the entire state space. However, differentiable DP is guaranteed to converge in iterations that are at most the length of the planning horizon while the VI module has to terminate in some fixed iterations to approximate the value iteration algorithm.

\subsubsection{Differentiable A* algorithm}
\label{subsubsec:diff_A}
Next, we present the more computationally efficient planning algorithm, differentiable A* algorithm, which does not have convolutional layers over the entire state space but only consider local convolutions over a subset of promising states. The key observation is that we can replace the optimal cost-to-go $V(x)$ from $x$ to $x_g$ in the differential dynamic programming algorithm with the $g$-values obtained from A* algorithm. Assuming that the cost of an optimal path from any state $x$ to any other state $x'$ is the same as that from $x'$ to $x$, we initialize A* from $x_g$ and search for the optimal path from the goal state $x_g$ to the current state $x_t$. When Algorithm~\ref{alg:2} terminates, $g(x)$ forms an upper bound for $V(x)$,
\begin{equation}
\begin{aligned}
g(x) = V(x) \; \forall x \in \text{CLOSED} \\
g(x) \geq V(x) \; \forall x \not\in \text{CLOSED}.
\end{aligned}
\end{equation}
The differentiability is again guaranteed in line 9 and 10 by implementing $g(f(x_{\tau},u_{\tau}))$ as the convolution of $g(x)$ with kronecker delta kernels $\delta(f(x_{\tau},u_{\tau})-x)$ accounting for the deterministic transitions from $x_{\tau}$ to $f(x_{\tau},u_{\tau})$ and min-pooling between the quantities $g(f(x_{\tau},u_{\tau}))$ and $ \hat{c}_t^{\theta}(x_{\tau},u_{\tau}) + g(x_{\tau})$. The convolutional operator is not applied to the entire state space but only locally on states popped from the OPEN list. Not only is differentiable A* algorithm more efficient than dynamic programming in obtaining the optimal cost-to-go $V(x_t)$ in the forward computation, it is also more efficient in constructing a correct gradient without backpropagating through multiple layers of convolutional and minpooling layers in the dynamic programming algorithm. The derivative of the $g$-values with respect to the cost function $\hat{c}^{\theta}_t$ has simple form as shown in Prop.~\ref{prop:1} and the proof is given in Appendix~\ref{app:a}. This property makes differentiable A* algorithm scale with the size of the environment. It is worth pointing out that if we start from some state $x_t \in$ CLOSED, the policy will give a small probability for $u_t$ if it leads to a next state outside CLOSED because $Q(x_t, u_t)$ is overestimated for such $(x_t, u_t)$, resulting in a ``safe'' planning trajectory that is unlikely to leave the CLOSED states.  \\ \\ 
\begin{algorithm}[ht]
\caption{Differentiable A* Algorithm}
\label{alg:2}
\begin{algorithmic}[1]
\STATE {\bfseries Input:} Current state $x_t$, goal state $x_g$, cost function $\hat{c}_t^{\theta}$, heuristic function $h$, deterministic transition $f$
\FUNCTION{Conv($g(x), \delta({f(x_{\tau},u_{\tau})} - x) $)}
    \STATE {\bfseries return} $\sum_{s=0}^{|\mathcal{X}-1|} \delta(f(x_{\tau}, u_{\tau})-s) g(s) $
\ENDFUNCTION
\STATE $g(x_g) = 0, \; g(x) = \infty \; \forall x \in \mathcal{X}$
\STATE OPEN $\gets \{x_g\}$, CLOSED $\gets \{\}$
\WHILE{$x_t \not\in $ CLOSED}
    \STATE Remove $x_{\tau}$ with smallest $f(x_{\tau}) = g(x_{\tau})+h(x_{\tau})$ from OPEN and insert $x_{\tau}$ in CLOSED
    \STATE $g(f(x_{\tau}, u_{\tau})) \gets \text{Conv}(g(x), \delta({f(x_{\tau},u_{\tau})} - x)), \; \forall u_{\tau} \in \mathcal{U}$
    \STATE $g(f(x_{\tau}, u_{\tau})) \gets \min\{g(f(x_{\tau}, u_{\tau})), \hat{c}_t^{\theta}(x_{\tau},u_{\tau}) + g(x_{\tau})\}, \; \forall u_{\tau}\in \mathcal{U}$ 
\ENDWHILE
\STATE $Q(x_t, u_t) \gets \hat{c}_t^{\theta}(x_t, u_t) + g(f(x_t, u_t))\; \forall u_t \in \mathcal{U}$
\STATE {\bfseries Output:} Policy $\pi_t^{\theta}(u_t|x_t) = \frac{\exp{\big(-Q(x_t, u_t)\big)}}{\sum_{u_t'\in \mathcal{U}}\exp{\big(-Q(x_t, u_t')\big)}}$
\end{algorithmic}
\end{algorithm}

\begin{proposition}
\label{prop:1}
For any current state $x_t \in \mathcal{X}$, let $g(x_t)$ be the cost of an optimal path from $x_t$ to the goal state $x_g \in \mathcal{X}$ as obtained in Alg.~\ref{alg:2}. We further assume that such optimal path is unique. Given any state $x \in \mathcal{X}$ and control $u \in \mathcal{U}$, the derivative $\frac{\partial g(x_t)}{\partial \hat{c}_t^{\theta}(x, u)}$ can be obtained as follows,
\begin{equation}
    \frac{\partial g(x_t)}{\partial \hat{c}_t^{\theta}(x, u)} = 
    \begin{cases}
        1, \text{ if } \hat{c}_t^{\theta}(x, u) \text{ is on the optimal path, } \\
        0, \text{ otherwise.}
    \end{cases}
\end{equation}
This derivative is the same as $\frac{\partial V(x_t)}{\partial \hat{c}_t^{\theta}(x, u)}$ by backpropagating through the differentiable dynamic programming algorithm.
\end{proposition}

\subsection{Cost learning via Differentiable Planning Model}
\label{subsec:cost_learning_planning}
Given a demonstration set $\mathcal{D}$, the policy $\pi_t^{\theta}(\cdot|x_t)$ is optimized by minimizing the cross-entropy loss $\mathcal{L}(\theta)$ defined in Problem~\ref{pb:2}. The computation graph in Figure~\ref{fig:approach} from learning a cost function from observations, to differentiable planning algorithms and to policy evaluation is differentiable end-to-end with respect to $\theta$ and stochastic gradient descent can be applied. The full algorithms for the training and testing phases (Figure~\ref{fig:approach}) are shown in Algorithms~\ref{alg:3} and~\ref{alg:4}.
\begin{algorithm}[ht]
\caption{Training: Learning the cost function parameters $\theta$ via differentiable planning}
\label{alg:3}
\begin{algorithmic}[1]
\STATE {\bfseries Input:} Demonstration set $\mathcal{D} = \crl{(x_{t,n},u_{t,n}^*,z_{t,n})}_{t=1, n=1}^{T_n,N}$
\WHILE{Policy not converged}
\STATE $\mathcal{L}(\theta) \gets 0$
\FOR{$n = 1:N$} 
    \FOR{$t = 1:T$}
        \STATE Estimate cost function $\hat{c}^{\theta}_{t,n}$ from current trajectory observation history $z_{1:t, n}$  as in Section~\ref{subsec:cost_repr}.
        \STATE Obtain stochastic policy $\pi^{\theta}_{t,n}$ from $\hat{c}_{t,n}^{\theta}$ as in Section~\ref{subsec:diff_plan}.
        \STATE $\mathcal{L}(\theta) \gets \mathcal{L}(\theta) -\log \pi^{\theta}_{t, n} (u_{t,n}^*|x_{t,n})$ 
    \ENDFOR
\ENDFOR
\STATE $\theta \gets \theta - \alpha \nabla \mathcal{L}(\pi_t)$
\ENDWHILE
\STATE {\bfseries Output:} Learned $\theta^*$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[ht]
\caption{Testing: output policy for a learned $\theta$}
\label{alg:4}
\begin{algorithmic}[1]
\STATE {\bfseries Input:} Start state $x_s$, goal state $x_g$, learned $\theta^*$ 
\STATE Current state $x_t \gets x_s$
\WHILE{$x_t \neq x_g$}
    \STATE Make an observation $z_t$
    \STATE Estimate cost function $\hat{c}^{\theta}_t$ from current trajectory observation history $z_{1:t}$ as in Section~\ref{subsec:cost_repr}.
    \STATE Obtain stochastic policy $\pi_t^{\theta}$ from $\hat{c}_t^{\theta}$ as in Section~\ref{subsec:diff_plan}
    \STATE Execute a control $u_t$ from policy $\pi_t^{\theta}(\cdot|x_t)$ and get next state $x_{t} \gets f(x_t, u_t)$
\ENDWHILE
\STATE {\bfseries Output:} Navigation succeeds or fails.
\end{algorithmic}
\end{algorithm}











==> tex/Evaluation.tex <==


\begin{figure}[t]
\centering
\begin{subfigure}[t]{.42\linewidth}
  \centering
  \includegraphics[width=\linewidth]{fig/VIN/Astar/path_succ.png}
  \caption{Predicted trajectory is optimal}
  \label{fig:sub1}
\end{subfigure}%
\hspace{1.6em}%
\begin{subfigure}[t]{.42\linewidth}
  \centering
  \includegraphics[width=\linewidth]{fig/VIN/Astar/path_fail.png}
  \caption{Predicted trajectory is suboptimal}
  \label{fig:sub2}
\end{subfigure}
%\vskip\baselineskip
\begin{subfigure}[t]{.45\linewidth}
  \centering
  \includegraphics[width=\linewidth]{fig/VIN/Astar/map_succ.png}
  \caption{Learned occupancy probability}
  \label{fig:sub1}
\end{subfigure}%
\hspace{1em}%
\begin{subfigure}[t]{.45\linewidth}
  \centering
  \includegraphics[width=\linewidth]{fig/VIN/Astar/map_fail.png}
  \caption{Learned occupancy probability}
  \label{fig:sub2}
\end{subfigure}
%\vskip\baselineskip
\begin{subfigure}[t]{.45\linewidth}
  \centering
  \includegraphics[width=\linewidth]{fig/VIN/Astar/g_succ.png}
  \caption{Learned optimal cost-to-go}
  \label{fig:sub1}
\end{subfigure}%
\hspace{1em}%
\begin{subfigure}[t]{.45\linewidth}
  \centering
  \includegraphics[width=\linewidth]{fig/VIN/Astar/g_fail.png}
  \caption{Learned optimal cost-to-go}
  \label{fig:sub2}
\end{subfigure}
\caption{Examples of successful navigation in 2D grid environment using \textbf{Ours-A*}. The first column is an example when the predicted path (in blue) has the same length as the optimal path (in red) and the second column is when the predicted path is suboptimal. The corresponding learned occupancy probability and optimal cost-to-go $V(x)$ are listed in the same row. Note that in (e) and (f), \textbf{Ours-A*} learns task-specific $V(x)$ by expanding only promising states while states in the white region are ignored.}
\label{fig:VIN}
\end{figure}


\section{Evaluation}
\label{sec:evaluation}
\textcolor{red}{The prior map log-odds and the parameter $L$ determines exploration}

We design experiments to answer the following questions:
\begin{enumerate}[nosep]
  \item  Does our model learn a cost function representation so that the expert policy is optimal? 
  \item Is the learned cost representation able to generalize to unseen environments.
  \item Does our model adapt to changing environments?
\end{enumerate}

\subsection{2-D Grid Navigation}
Think of the metrics to report here, how to log data: $\theta$, $lr$, epochs, training loss, training error, validation accuracy, test accuracy.

\begin{center}
\begin{tabular}{|c|c|c|c|}
    \hline
    Models & Environment & Succ. rate & Traj. diff. \\
    \hline
    \textbf{VIN} & Fully obs. & 95.12 \% & 0.264 \\
    \hline
    \textbf{Ours-A*} & Fully obs. & 100 \% &  0.000 \\
    \hline 
    \textbf{Ours-A*} & Partially obs. & 95.23 \% & 0.241 \\
    \hline
    \textbf{Ours-A*} & Partially obs. w/ noise & 95.96\% & 0.263 \\
    \hline
\end{tabular}
\end{center}

The first experiment evaluates whether the models can make successful navigation in a 2D gridworld environment with randomly generated obstacles. Although optimal controls can be computed in this simple domain, we are interested in evaluating our cost learning from differentiable planning model to show that the learned cost function can be generalized to successful navigation in novel, unseen environments. We consider the fully observable environment where the observation is the map and the expert controls are calculated by Dijkstra's algorithm.

We compare three models: \textbf{VIN}, \textbf{Ours-DP} and \textbf{Ours-A*}. We follow the original \textbf{VIN} architecture~\cite{Tamar_VIN16} and $k=20$ layers of value iterations. For \textbf{Ours-DP}, we use the log-odds cost representation described in Sec.~\ref{sec:cost_rep} with differentiable dynamic programming algorithm described in Sec.~\ref{sec:diff_dp}. The number of dynamic programming iterations is set to $k=20$ as well. \textbf{Ours-DP} is an extension of \textbf{VIN} on the deterministic finite horizon shortest path problem and we consider \textbf{Ours-DP} as the baseline. \textbf{Ours-A*} uses the same log-odds cost representation but uses the differentiable A* algorithm described in Sec.~\ref{sec:diff_A} as the planning model.

In Fig.~\ref{tb:1}, we present the generalization performance on a test set consisting $N=1000$ maps with randomly generated obstacle configurations, starts and goals. In each map, a robot iteratively queries the models for a control prediction at the current state and move to the corresponding next state to form a trajectory. A trajectory is regarded as successful if the robot finds a path from start to goal without collision even if it is not optimal. The trajectory length difference is calculated between the rolled-out trajectory formed by the models and the shortest path calculated by Dijkstra's algorithm. Our results show that \textbf{Ours-A*} can be generalized to successful navigation in unseen 2D grid environments indicating a correct cost function representation is learned. Examples of successful trajectories and the learned occupancy probability and values are shown in Fig.~\ref{fig:VIN}.


\begin{figure}
\begin{minipage}{.48\linewidth}
\centering
\resizebox{\linewidth}{!}{\begin{tabular}{ |c|c|c| }
    \hline
    Models  & Succ. rate & Traj. diff. \\
    \hline
    \textbf{VIN} & 95.12 \% & 0.264 \\
    \hline
    \textbf{Ours-DP} & 100 \% & 0.211 \\
    \hline
    \textbf{Ours-A*} & 100 \% &  0.183 \\
    \hline 
\end{tabular}}
\caption{Test set performance of VIN and our models.}
\label{tb:1}
\end{minipage}%
\hfill%
\begin{minipage}{.5\linewidth}
\centering
\includegraphics[width=\linewidth]{fig/Dyna/cum_reward.png}
\vspace{-5ex}
\caption{Average performance of \textbf{Dyna-Q} and \textbf{Ours-A*}}
\label{fig:dyna_cum_reward}
\end{minipage}
\end{figure}

\begin{figure}[t]
\centering
\begin{subfigure}[b]{.44\linewidth}
  \centering
  \includegraphics[width=\linewidth]{fig/Dyna/map_before.png}
  \caption{Dyna maze before change}
\end{subfigure}%
\hspace{1em}%
\begin{subfigure}[b]{.43\linewidth}
  \centering
  \includegraphics[width=\linewidth]{fig/Dyna/map_after.png}
  \caption{Dyna maze after change}
\end{subfigure}
\vspace{-2ex}
\caption{The Dyna blocking maze environment. We consider episodic tasks of navigation from the start (blue) to goal (red). The environment is divided by a wall in the middle. The right door is open for the first 1000 steps, then the left door is open until 3000 steps. \textbf{Ours-A*} finds the new configuration consistently while \textbf{Dyna-Q} frequently does not find the new path.}
\label{fig:Dyna_maze}
\end{figure}


%\begin{table}[ht]
%\centering
%\begin{tabular}{ |c|c|c|c|c| }
%    \hline
%    Models & Training loss & Validation acc & Success rate & Traj. diff. \\
%    \hline
%    VIN & 0.2181 & 93.69 \% & 95.12 \% & 0.264 \\
%    \hline
%    Ours-DP & 0.4684 & 83.32\% & 100 \% & 0.211 \\
%    \hline
%    Ours-A* & 0.4195 & 83.66\% & 100 \% &  0.183 \\
%    \hline 
%\end{tabular}
%\caption{Prediction performance of our models and VIN on the training and test set.}
%\label{tb:1}
%\end{table}





\subsection{Online Learning in Changing Environments}
In this experiment, we compare \textbf{Ours-A*} with the \textbf{Dyna-Q} algorithm in a changing environment. We demonstrate how our models efficiently adapts to environment changes. Consider an episodic task in a Dyna blocking maze gridworld~\cite{Sutton_RL18} with fixed start and goal in Fig.~\ref{fig:Dyna_maze}. The gridworld is separated by a wall with the right door open in the first phase and left open in the second. The robot can move to one of its 8 adjacent states if it is not an obstacle. The robot receives a reward of 1 if it reaches the goal and 0 otherwise in each step. The robot observation is the occupancy label only at the next state that it plans to arrive at. We consider the \textbf{Dyna-Q} algorithm~\cite{Sutton_RL18} for comparison, which interleaves between learning with real experience and planning with simulated experience. Planning with simulated experience using a learned model is similar to expanding nodes in \textbf{Ours-A*}. To set up a fair comparison, we set the number of planning steps between each real transition in \textbf{Dyna-Q} to be at least the number of nodes expanded by the A* algorithm in our model. The expert control $u^*$ for \textbf{Ours-A*} is given by an optimal planner on the map observed so far, and the unobserved regions are assumed to be free. 

Fig.~\ref{fig:dyna_cum_reward} shows the performance of the \textbf{Dyna-Q} and \textbf{Ours-A*} averaged over 10 trials. The higher the slope of the curve, the better the model is in finding a shortest path to goal. \textbf{Ours-A*} plateaus when the environment changes but quickly adapts to the new configuration afterwards. The \textbf{Dyna-Q} model is comparable to \textbf{Ours-A*} before the map changes, but struggles to learn the new configuration using random exploration and therefore the slope of the average reward is lower. Planning with simulated experience does not help in this case if the new configuration is not encountered when interacting with the real environment. Figure~\ref{fig:Dyna} shows the episodes before and after the map changes. \textbf{Ours-A*} quickly adapts to the new configuration by learning the new occupancy probability and consistently finds the new path afterwards. \\ \\



\begin{figure}[h]
\centering
\begin{subfigure}[t]{.45\linewidth}
  \centering
  \includegraphics[width=\linewidth]{fig/Dyna/value_before.png}
  \caption{Optimal cost-to-go in log scale for the last episode before map changes}
\end{subfigure}%
\hspace{1em}%
\begin{subfigure}[t]{.45\linewidth}
  \centering
  \includegraphics[width=\linewidth]{fig/Dyna/path_before.png}
  \caption{Policy trajectory for the last episode before map changes}
\end{subfigure}
\begin{subfigure}[t]{.45\linewidth}
  \centering
  \includegraphics[width=\linewidth]{fig/Dyna/value_after.png}
  \caption{Optimal cost-to-go in log scale for the first episode after map changes}
\end{subfigure}%
\hspace{1em}%
\begin{subfigure}[t]{.45\linewidth}
  \centering
  \includegraphics[width=\linewidth]{fig/Dyna/path_after.png}
  \caption{Policy trajectory for the first episode after the map changes}
\end{subfigure}
\begin{subfigure}[t]{.45\linewidth}
  \centering
  \includegraphics[width=\linewidth]{fig/Dyna/value_after2.png}
  \caption{Optimal cost-to-go in log scale for the second episode after the map changes}
\end{subfigure}%
\hspace{1em}%
\begin{subfigure}[t]{.45\linewidth}
  \centering
  \includegraphics[width=\linewidth]{fig/Dyna/path_after2.png}
  \caption{Policy trajectory for the second episode after the map changes}
\end{subfigure}
\caption{\textbf{Ours-A*} model performance for the last episode before map changes in the first row, first and second episodes after map changes in the second and third rows. The first column shows the optimal cost-to-go $V(x)$ in log scale and the second column shows the policy trajectory on the learned occupancy probability map. Note that Our-A* does not expand every state while quickly adapts to the new configuration.}
 \label{fig:Dyna}
\end{figure}







==> tex/old/Abstract.tex <==
\begin{abstract}
This paper focuses on Inverse Reinforcement Learning (IRL) in partially observable environments.
That is, learning cost functions that capture expert-demonstrated behavior.
A na\"ive application of IRL algorithms designed for fully observed environments is
inefficient because they perform redundant computations on unexplored regions of the environment.
To address this issue, we make two contributions.
Firstly, we propose an efficient planning algorithm that updates cost-to-go
estimates only on a subset of promising states.
Furthermore, we efficiently back-propagate the gradients by computing the closed-form
gradient of cost-to-go with respect to the learned cost-function.
Secondly, we propose a learnable cost-function representation that works with
partially observable environments and integrate it with the planning algorithm
in an end-to-end trainable framework.
We train our model on trajectories generated by shortest-path expert in 2D grid
environments as well as the CARLA simulator~\cite{Dosovitskiy_CARLA17}.
Our experiments show that we match or exceed the accuracy of the baseline
algorithm~\cite{Ziebart_MaxEnt08}, while substantially improving in terms of
efficiency.
\end{abstract}

==> tex/old/Approach_1_Cost.tex <==
\section{Cost Function Representation}
\label{sec:cost_rep}

\begin{figure}[t]
  \centering
  %\includegraphics[width=\linewidth]{fig/CostNeuralNet}
  \def\svgwidth{\linewidth}
  \input{fig/CostNeuralNet.pdf_tex}
  \caption{Neural network model of a cost function. A recurrent neural network, parameterized by $\bftheta_1$, takes in sequential observations $\bfz_{1:t}$ and outputs a latent map representation $m$. A convolutional neural network, parameterized by $\bftheta_2$, extracts features from the map state $m$ to specify the cost $c_t$ at a given robot state-control pair $(\bfx,\bfu)$. The learnable parameters are $\bftheta = \crl{\bftheta_1, \bftheta_2}$.}
  \label{fig:cost_neural_net}
\end{figure}



\subsection{Cost Model on Partially Observable Environments}
\label{sec:general_cost}

Our desired cost function naturally decomposes into two stages.
The first stage, called the \textit{Map encoder}, uses the observation history
$\bfz_{1:t}$ to estimate a latent environment state $m$.
Any modeling choice for this stage will require to
take an arbitrary length sequential input and output fixed size latent state estimate,
for example, a recurrent neural network (RNN)~\cite{Goodfellow-et-al-2016}.
The second stage, called the \textit{Cost on map model}, uses $m$ to define a cost estimate at given state-control pairs $(\bfx,\bfu)$.
This stage can be represented by many different models that converts
multi-dimensional latent state to a real cost estimate.
For representations like occupancy grid mapping
The second stage can be represented using a
convolutional neural network (CNN) with parameters $\bftheta_2$.
The complete model, combining recurrent estimation of the environment state, followed by feature extraction to define the cost at $(\bfx,\bfu)$ is illustrated in Fig.~\ref{fig:cost_neural_net}.
Since this model is differentiable, its parameters $\bftheta = \{\bftheta_1, \bftheta_2\}$ can be optimized.


% The RNN provides a differentiable model of the dependence of the sequential observations on the underlying environment state. 
%Learning a cost function from observations can be encoded as a neural net in general as shown in Figure~\ref{fig:cost_neural_net}. We first train a recurrent neural net (RNN) with parameters $\theta_1$ that consumes the high-dimensional observations sequentially and outputs a low-dimensional latent environment representation $\hat{m}_t$. The RNN models the dependence of the sequential observations on the underlying state of the environment. The idea of extracting occupancy information from observations and keeping track of an internal latent map representation is also explored in~\cite{Gupta_CMP17, Oh_ActPred15}. \TW{~\cite{Khan_MACN_ICLR18} does not have this RNN strucuture. It processes the observations as in VIN (the CONV block in Fig. 3). The controller is LSTM though.} 


%The latent map representation $\hat{m}_t$ is fed into a convolutional neural net (CNN) with parameters $\theta_2$, along with state $x$ and control $u$. It encodes spatial feature from the latent map to produce a cost function $\hat{c}_t^{\theta}$ for planning. With the implementation of neural nets as cost function representation, we emphasize that the output cost function $\hat{c}_t^{\theta}$ is differentiable with respect to the network parameters $\theta = \{\theta_1, \theta_2\}$. We will later learn the parameters $\theta$ as part of the policy learning process. 

\subsection{Occupancy-based Map encoder}
\label{sec:occupancy_cost}
\TW{I abandoned the previous version using the forward observation model because $p(z_t[i] \mid x_t, m[j])$ is hard to model. $z_t[i]$ depends on not just a single cell $m[j]$ but probably the full map $m$. In this version I will write the log odds in terms of the inverse observation model $p(m[j] \mid x_t, z_t[i])$.}
In this section, we propose an instantiation of the general neural network model specific to modeling occupancy in robot navigation tasks with lidar observations.
The idea of extracting occupancy information from observations in the form of a
latent map representation has been explored in~\cite{Gupta_CMP17, Oh_ActPred15}.
Suppose that the robot is equipped with a lidar for range and bearing measurements with maximum range $d_{max}$ and the range measurement is corrupted by noise.
\TW{Shall we have Gaussian noise explicitly?}
We discretize $\mathcal{X}$ into $N$ cells and the robot's goal is to maintain
the probability distribution $p(m \mid \bfx_{1:t}, \bfz_{1:t})$ of the $N$
independent Bernoulli random variables of $m$ to approximate the true map $m^*
\in \{-1,1\}^N$.
See Fig.~\ref{fig:map_and_obs} for an example of such lidar observations and
occupancy map.
\TW{Does this figure illustrates how lidar observation is made? 
Shall I show the ray instead of just the endpoint of the ray? 
Shall I show the ones that reach $y_{max}$ and do not hit the obstacle?}
We can write the posterior of $m$ in terms of the product of occupancy
probability of each cell,
\begin{equation}
p(m \mid \bfx_{1:t}, \bfz_{1:t}) = \prod_{j=1}^N p(m[j] \mid \bfx_{1:t}, \bfz_{1:t}).
\end{equation}
Estimating the occupancy probability of each cell $m[j]$ is a filtering problem and can be solved by the Bayes filter~\cite[Ch 9.2]{Thrun_PR05}. Define the log odds ratio of occupancy as 
\begin{equation}
\lambda_t(m[j]) := \log \frac{p(m[j]=1 \mid \bfx_{1:t}, \bfz_{1:t})}{p(m[j]=-1 \mid \bfx_{1:t}, \bfz_{1:t})},
\end{equation}
which can be updated recursively as
\begin{equation}
\begin{aligned}
\label{eq:log_odds_update_rule}
\lambda_t(m[j]) &= \lambda_{t-1}(m[j]) + \log \frac{p(m[j]=1 \mid \bfx_t, \bfz_t)}{p(m[j]=-1 \mid \bfx_t, \bfz_t)} \\
    & \quad - \log\frac{p(m[j]=1)}{p(m[j]=-1)}.
\end{aligned}
\end{equation}
The posterior can be recovered from the log odds ratio through the sigmoid function
\begin{equation}
\begin{aligned}
p_t(m[j]) := p(m[j]=1 \mid \bfx_{1:t}, \bfz_{1:t}) = \sigma(\lambda_t(m[j])).
\end{aligned}
\end{equation}
Assuming that the priors of the map are equal,
\begin{equation}
\label{eq:map_prior}
\log\frac{p(m[j]=1)}{p(m[j]=-1)} = 0,
\end{equation}
%
we are left with the log odds of the inverse observation model for each
additional time-step.
Let $z_t[k]$ be the $k$\suth{} beam of the lidar scan $\bfz_t$, 
and assume the beams of $\bfz_t$ are independent, we can
%
%\begin{equation}
%\log \frac{p(m[j]=1 \mid \bfx_t, \bfz_t)}{p(m[j]=-1 \mid \bfx_t, \bfz_t)} = \sum_{k=1}^K \log \frac{p(m[j]=1 \mid \bfx_t, z_t[k])}{p(m[j]=-1 \mid \bfx_t, z_t[k])},
%\end{equation}
%
simplify the log odds update rule in Eqn~\eqref{eq:log_odds_update_rule} as 
%
\begin{equation}
\label{eq:simplified_log_odds}
\lambda_t(m[j]) = \lambda_{t-1}(m[j]) + \sum_{k=1}^K \log \frac{p(m[j]=1 \mid \bfx_t, z_t[k])}{p(m[j]=-1 \mid \bfx_t, z_t[k])} .
\end{equation}
%

\paragraph{Inverse observation model}
\VD{Tianyu: I prefer a sigmoid function that
  depends upon the length of laser obsservation $z_t[k]$.
  That also simplifies the different cases into single smooth function.
  If you prefer your model, I have cleaned up the writing a bit. You can
  uncomment it back too.}
Next, we discuss the parameterization of
the inverse observation model for noisy observations $z_t[k]$.
Let $d(\bfx_t, m[j])$ be the distance between the robot pose $\bfx_t$ and the
center of mass of cell $m[j]$.
We assume that the cells that are not in the direction of $z_t[k]$ or beyond
distance $d_{max}$ are independent of $z_t[k]$.
The log-odds for such independent cell-observation pairs is zero and does not
contribute to Eqn~\eqref{eq:simplified_log_odds}.

%\input{tex/Approach_1_Cost_ThreeCaseModel}
\input{tex/Approach_1_Cost_SigmoidModel}

The logistic regression model in Eqn~\eqref{eq:sigmoid_inv_obs_model_occ} and~\eqref{eq:sigmoid_inv_obs_model_free} suggests that a more expressive multi-layer neural network can be applied,
\begin{equation}
\label{eq:sigmoid_inv_obs_model}
p(m[j] \mid \bfx_t, z_t[k]) = \sigma(m[j]\textbf{NN}(z_t[k], d(\bfx_t, m[j]));\bftheta_1). 
\end{equation}
This model would be flexible for more complicated observations, such as images, from which it will be difficult to extract occupancy information. The log odds ratio for such inverse observation model can be written as 
\begin{equation}
\label{eq:general_log_odds}
\log \frac{p(m[j]=1 \mid \bfx_t, z_t[k])}{p(m[j]=-1 \mid \bfx_t, z_t[k])} = \textbf{NN}(z_t[k], d(\bfx_t, m[j]);\bftheta_1) ,
\end{equation}
which suggests that we can train a neural network to predict the log odds ratio
of the inverse observation model given noisy observations $\bfz_t$ at robot pose
$\bfx_t$. For the simple models in Eqn~\eqref{eq:sigmoid_inv_obs_model_occ}
and~\eqref{eq:sigmoid_inv_obs_model_free}, Eqn~\eqref{eq:general_log_odds}
simplifies to $\theta_{k,occ}(-\delta z_t[k] + \epsilon)$.








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{No noise in measurement}\TW{This is the observation model implemented in the code}
%The observation model can be simply parameterized by a sigmoid function indicating how much confidence we have in the occupancy measurement,
%\begin{equation}
%     p(z_t[i] \mid x_t, m[j]) = 
%     \begin{cases}
%     \sigma(m[j] \theta_1),& z_t[i] = y_i(x_t, m[j])\\
%     \sigma(-m[j] \theta_1), & z_t[i] > y_i(x_t, m[j])
% \end{cases} \label{eq:observation_model}\\
%\end{equation}

% Model version 3
%\begin{multline}
%    p(z_t[i] \mid x_t, m[j]) = 
%    \\
%    %\begin{cases}
%    \frac{\sigma(m[j])}{\sqrt{2\pi}\theta_1[1]}
%    \exp\left(
%    - \frac{(z_t[i] -  y_i(x_t, m[j]))^2}
%    {2(\theta_1[1])^2}
%    \right)%, & m[j] \ge 0
%    \\ 
%    +
%    (\theta_{1}[2]\mathbbm{1}_{z_t[i] = y_{\text{max}}}
%    + (1 - \theta_{1}[2])\mathbbm{1}_{z_t[i] < y_{\text{max}}})
%    (1-\sigma(m[j])),% & m[j] < 0
%  %\end{cases}.
%\label{eq:observation_model}
%\end{multline}

%Note that the cells that are not in the direction of the
%$i$\suth lidar beam or ones beyond the lidar range, $y_i(x_t, m[j]) >
%y_{\text{max}}$
%are independent of the laser observation. This sigmoid model is used in occupancy mapping in robotics~\cite[p156]{Thrun_PR05} and is the same discriminative model used in logistic regression. The latter suggests that an even more expressive model can be obtained by using a multi-layer convolutional neural network with a sigmoid output,\TW{I am not sure if this CNN is correct}
%\begin{equation}
%\label{eq:cnn_observation_model}
%    p(z_t[i] \mid x_t, m[j]) = \sigma\Big(m[j]\textbf{CNN}(z_t[i], x_t, m[j]; \theta_1)\Big)
%\end{equation}
%This model would be flexible for more complicated observations, such as images, where it is difficult to model occupancy information from observations. Since the map $m$ is assumed binary, we can work with the log-odds ratio of the observation model in~\eqref{eq:cnn_observation_model}:
%\begin{equation}
%\label{eq:observation_log_odds}
%    \log \frac{p(z[i] \mid x_t, m[j]=1)}{p(z[i] \mid x_t, m[j]=-1)} = \textbf{CNN}(z_t[i], x_t, m[j]; \theta_1).
%\end{equation}
%For the simple observation model in~\eqref{eq:observation_model}, eqn~\ref{eq:observation_log_odds} is just $\theta$ for the cell where the lidar hits the obstacle and $-\theta$ for the cells along the ray of $z[i]$ until it hits the obstacle.%

%\subsubsection{Noisy measurements}\TW{This is the observation model with Vikas's help}
%In this section we derive the log-odds ratio for a noisy lidar observation model proposed in~\cite{Thrun_PR05}. Instead of the simple sigmoid function in~\eqref{eq:observation_model}, we model the distribution of the lidar measurement $z[i]$ as a Gaussian around the true range $y_i(x_t, m[j])$ if the cell is occupied $m[j] = 1$ and uniform over the support ($0 \leq z[i] \leq y_{max}$) if it is free $m[j] = -1$,
%\begin{equation}
%\begin{aligned}
%    &p(z[i] \mid x_t, m[j]) = \\
%    & \; \begin{cases}
%    \mathbbm{1}_{z[i] \leq y_{max}} \eta_1 \exp\big(-(z[i] - y_i(x_t, m[j]))^2 / 2\sigma^2\big) \\ 
%    \quad \quad \quad \text{ if } m[j] = 1 \\
%    \mathbbm{1}_{z[i] \leq y_{max}} \eta_2 \text{ if } m[j] = -1
%    \end{cases}
%\end{aligned}
%\end{equation}
%where $\eta_1, \eta_2$ are normalization constants. The log-odds ratio of the observation likelihood is 
%\begin{equation}
%\begin{aligned}
%& \log \frac{p(z[i] \mid x_t, m[j]=1)}{p(z[i] \mid x_t, m[j]=-1)} \\
%& \;\; = \log \frac{\eta_1}{\eta_2} - \frac{\big(z[i] - y_i(x_t, m[j])\big)^2}{2\sigma^2}
%\end{aligned}
%\end{equation}



\begin{figure}[t]
\centering
\includegraphics[width=.48\textwidth]{fig/lidar_observation.png}
\caption{A navigation scenario of a robot (green) in a 2D grid environment. The true environment on the left is a $16\times 16$ grid in which black regions are obstacles and white regions are free space. The lidar scans in red has maximum range $y_{max} = 2.5$ and can reveal occupancy labels of nearby cells while the remaining part of the environment (grey regions) is not observable.}
 \label{fig:map_and_obs}
\end{figure}

%Given a history of observations $z_{1:t}$, the log-odds ratio of the occupancy probability of the $j$\suth cell can be obtained recursively using Bayes rule as a sum of the log-odds ratio of the observation model over time:
%\begin{equation}
%\begin{aligned}
%&\lambda(m[j] \mid x_{1:t}, z_{1:t}) := \log \frac{p(m[j]=1 \mid x_{1:t}, z_{1:t})}{p(m[j]=-1 \mid x_{1:t} z_{1:t})} \\
%& \quad = \sum_{i}\log \frac{p(z_t[i] \mid x_t, m[j] = 1)}{p(z_t[i] \mid x_t, m[j] = -1)} \\
%& \quad \quad + \log \frac{p(m[j]=1 \mid x_{1:t-1}, z_{1:t-1})}{p(m[j]=-1 \mid x_{1:t-1}, z_{1:t-1})} \\
%& \quad = \lambda(m[i]) + \sum_{\tau=1}^t \textbf{CNN}(z_t[i], x_t, m[j];\theta_1)
%\end{aligned}
%\end{equation}
%The log-odds ratio $\lambda(m[j] \mid x_{1:t}, z_{1:t})$ for $i=1,\ldots,N$ can
%be regarded as the hidden state $h_t$ in Fig.~\ref{fig:cost_neural_net} and
%accumulates $\textbf{CNN}(z_t[i], x_t, m[j];\theta_1)$
%% (or simply $\pm \theta_{1}$ in the case of direct occupancy measurements)
%for each new observation $z_t$. Finally, the output is the probability density function $p_t^{\theta_1}(m)$, which can be recovered from the log-odds $\lambda(m[j] \mid x_{1:t}, z_{1:t})$ by
%\begin{equation}
%p_t^{\theta_1}(m) = \prod_{j=1}^N \sigma\Big(m[j]\lambda(m[j] \mid x_{1:t}, z_{1:t})\Big)\;.
%\end{equation}
%We emphasize that $p_t^{\theta_1}(m)$ is a function of $\theta_1$ through $\lambda(m[j] \mid x_{1:t}, z_{1:t})$ and is differentiable with respect to $\theta_1$.

\subsection{Cost on map model}
\textit{Cost on map model} maps the latent occupancy state $m$ to a cost
function $c_t$.
As suggested by~\cite{Wulfmeier_DeepMaxEnt15}, we can train deep neural networks
to model the true underlying cost $c^*$ which has complex interacting structure
over the feature representation (the occupancy probability $p_t(m)$ in our
case).
Several CNN architectures are proposed in~\cite{Wulfmeier_DeepMaxEnt15} and they
can be applied here with proper modification of padding size and channels.
However, we can design a simpler cost function since we explicitly model
$p_t(m)$ for navigation tasks in grid environments that look for shortest paths
and avoid collisions.
Let $s$ and $l$ be a small and a large positive parameter respectively.
We can model the cost of applying control $\bfu$ in robot state $\bfx$ for a given map $m$ as:
\begin{equation}
c(\bfx,\bfu)\!:=\!
    \begin{cases}
    s, \; & \text{if} \: m[\bfx] \!=\! -1 \text{ and } m[f(\bfx, \bfu)] \!=\! -1\\
    l, & \text{if } m[\bfx] \!=\! 1 \text{ or } m[f(\bfx, \bfu)] \!=\! 1 
    \end{cases}
\end{equation}
Since $m$ is unknown, we use the estimated occupancy probability $p_t(m)$ to compute the expectation of $c(\bfx,\bfu)$ over $m$:
\begin{equation}
\begin{aligned}
\label{eq:chat}
c_t(\bfx, \bfu) &:= \mathbb{E}_{m} [c(\bfx, \bfu)] \\
&= p_t(m[\bfx])p_t(m[f(\bfx, \bfu)]) \times s\\
                          &+\prl{1-p_t(m[\bfx])p_t(m[f(\bfx, \bfu)])} \times l \; .
\end{aligned}
\end{equation}
Our cost-encoding layer has parameters $\bftheta_2 := (s,l)$ and its output $c_t(\bfx, \bfu)$ is differentiable with respect to $\bftheta_2$ and $\bftheta_1$ through $p_t(m)$. 





%Of course, a more complex neural network model could be used to represent $\hat{c}_t^{\theta}(x, u)$ in terms of $p_t^{\theta_1}(m)$.








%As a specific instantiation of the general problem setting stated above, we choose to demonstrate the idea of learning cost functions through differentiable planning model by considering navigation tasks in a 2D grid cells. Let $m^* \in \{0, 1\}^n$ be a true occupancy map, so $m^*[x] = \{0,1\}$ is the occupancy label at state $x$. The robot receives binary observations $z_t = H(x_t) m^*$, where $z_t \in \{0, 1\}^n$ and the diagonal matrix $H(x_t) \in \{0,1\}^{n \times n}$ consists of ones for observable states and zeros for unobservable states, capturing the local field of view of the robot at $x_t$. An example of such occupancy map and robot observation is shown in Figure~\ref{fig:map_and_obs}.

%Next, we show a specific occupancy-based design of the cost function representation for navigation in 2D grid environments. Instead of using a standard RNN model, we accumulate the log-odds ratio of the occupancy probability of each cell. Let $\hat{m} \in \{0, 1\}^n$ be the map occupancy estimate which is a collection of $n$ independent Bernoulli random variables. The probability density of $\hat{m}$ can be updated via an observation model which is a sigmoid function parameterized by $\theta_1$, indicating how much we trust the observation measurements,
%\begin{equation}
%\begin{aligned}
%p(z_t|\hat{m};\theta_1) &:= 
%\begin{cases}
%    \sigma(\theta_1),& \text{if } z_t = \hat{m}\\
%    \sigma(-\theta_1), & \text{if } z_t \neq \hat{m}
%\end{cases} \\
%&= \sigma((2z_t-1)(2\hat{m}-1)\theta_1) \;.
%\end{aligned}
%\end{equation}
%Note that we drop the argument $x$ for brevity since the random variables $\hat{m}[x]$ are independent. We choose the sigmoid observation model demonstrate the feasibility of the model in the 2D grid environment and it can be replace by a CNN if the observations are more complicated. We can simplify the log-odds ratio of the observation model as
%\begin{equation}
%\ln \frac{p(z_t|\hat{m}=1)}{p(z_t|\hat{m}=0)} = (2z_t-1)\theta_1 \;.
%\end{equation}
%Given a history of observations $z_{1:t}$, the robot estimates the log-odds ratio $\lambda \in \mathbb{R}^n$ of the occupancy probability, which can be decomposed using Bayes rule as a sum of the log-odds ratio of the observation model over time,
%\begin{equation}
%\begin{aligned}
%\lambda(\hat{m} \mid z_{1:t}) &:= \ln \frac{p(\hat{m}=1 \mid z_{1:t})}{p(\hat{m}=0 \mid z_{1:t})} \\
%&= \lambda(\hat{m}) + \sum_{\tau=1}^t (2z_{\tau}-1)\theta_1
%\end{aligned}
%\end{equation}
%with some prior $\lambda(\hat{m})$. The log-odds ratio $\lambda(\hat{m} \mid z_{1:t})$ can be regarded as the hidden state $h_t$ in Figure~\ref{fig:cost_neural_net} and accumulates $(2z_t-1)\theta_1$ for each new observation $z_t$. Finally, the output is the probability density function of the map estimate $\hat{m}$, which can be recovered from the log-odds $\lambda(\hat{m} \mid z_{1:t})$ by 
%\begin{equation}
%\begin{aligned}
%p_t^{\theta_1}(\hat{m}) &:= p(\hat{m} = 0 \mid z_{1:t}) \\
%              &= \frac{1}{1+\exp(\lambda(\hat{m} \mid z_{1:t}) )} \;.
%\end{aligned}
%\end{equation}
%We would like to emphasize that $p_t^{\theta_1}(\hat{m})$ is a function of $\theta_1$ through $\lambda(\hat{m} \mid z_{1:t})$ as we require that the output is differentiable with respect to $\theta_1$.

%Instead of implementing a CNN block in Figure~\ref{fig:cost_neural_net}, we adopt an induced cost function from map estimate. Implementing a CNN is not necessary as we explicitly model the occupancy probability of each cell in the 2D environment while in the general case we do not know what the hidden state $h_t$ represents. The cost function can be induced from the map estimate $\hat{m}$ as follows. Let the actual cost of each control be
%\begin{equation}
%c(x_t,u_t):=
%    \begin{cases}
%    s, \; & \text{if} \: \hat{m}[x_t] = 0 \text{ and } \hat{m}[f(x_t, u_t)] = 0\\
%    l, & \text{if } \hat{m}[x_t] = 1 \text{ or } \hat{m}[f(x_t, u_t)] = 1 
%    \end{cases}
%\end{equation}
%where $s$ and $l$ are some small and large positive constants (for example, $s=\lVert x_t-f(x_t, u_t) \rVert_2 $ and $l = 100s$\TW{This looks too arbitrary. Also $x_t$ is not the coordinate of the grid}). The estimated cost function $\hat{c}^{\theta}_t$ is the expected value of $c$,
%\begin{equation}
%\begin{aligned}
%\label{eq:chat}
%\hat{c}_t^{\theta}(x_t, u_t) &= \mathbb{E}_{\hat{m}} [c(x_t, u_t)] \\
%&= p_t^{\theta_1}(\hat{m}[x_t])p_t^{\theta_1}(\hat{m}[f(x_t, u_t)]) \times s + \\
%                          &\Big(1-p_t^{\theta_1}(\hat{m}[x_t])p_t^{\theta_1}(\hat{m}[f(x_t, u_t)])\Big) \times l \; .
%\end{aligned}
%\end{equation}
%Note that the output $\hat{c}_t^{\theta}(x_t, u_t)$ is differentiable with respect to $\theta_1$ through $p_t^{\theta_1}(\hat{m})$.

%In summary, we design a cost function representation which is differentiable with respect to its parameters in 2D grid environments. The cost function is induced from the occupancy probability of the cells which is updated by the log-odds ratio of the parameterized observation likelihood. 



==> tex/old/Approach_1_Cost_SigmoidModel.tex <==
We model the occupancy of the cell $m[j]$ as a truncated sigmoid around true
distance $d(\bfx_t, m[j])$,
%
\begin{multline}
  p(m[j] = 1 | \bfx_t, z_t[k]) =
  \\
  \begin{cases}
    \sigma \left(\theta_{k,occ}(-\delta z_t[k])\right)
    & \text{ if } \delta z_t[k] \geq -\epsilon \\
    0.5 & \text{ otherwise }
    \end{cases}
    \label{eq:sigmoid_inv_obs_model_occ},
\end{multline}
%
where $\delta z_t[k] \defeq  z_t[k] - d(\bfx_t,m[j])$,
$\epsilon$ denotes the distance threshold of the influence of laser
observation on the cells around the point of reflection,
and $\theta_{k,occ}$ is a learnable positive parameter.
Since $\sigma(-x) = 1-\sigma(x)$ and $m[j]$ is binary random variable, we
can re-write Eqn~\eqref{eq:sigmoid_inv_obs_model_occ} as
%
\begin{multline}
  p(m[j] | \bfx_t, z_t[k]) =
  \\
  \begin{cases}
    \sigma \left(m[j]\theta_{k,occ}(-\delta z_t[k])\right)
    & \text{ if } \delta z_t[k] \geq -\epsilon \\
    0.5 & \text{ otherwise }
    \end{cases}
    \label{eq:sigmoid_inv_obs_model_free},
\end{multline}
%

==> tex/old/Approach_1_Cost_ThreeCaseModel.tex <==
We consider parameterization in three separate cases. First, when the laser-scan
seems to have passed through the cell $z_t[k] > d(\bfx_t, m[j]) + \epsilon$,
where $\epsilon$ denotes the distance threshold on influence of the laser
observation on the cells around the point of reflection.
Second, when the laser-scan seems to have hit the desired cell
$|z_t[k]-d(\bfx_t, m[j])| \leq \epsilon$. And lastly, when the laser-scan seems
to have hit something well before the cell $z_t[k] < d(\bfx_t, m[j]) - \epsilon$.


\textit{Case 1:} $z_t[k] > d(\bfx_t, m[j]) + \epsilon$. Since the laser-scan passed
through the cell, it is more likely to be free than not. For a large positive
learnable parameter $\theta_{k,free}$, we have
%
\begin{equation}
\begin{aligned}
p(m[j] = 1 \mid \bfx_t, z_t[k]) &= \sigma(\theta_{k, free}) \\
p(m[j] = -1 \mid \bfx_t, z_t[k]) &= 1 - \sigma(\theta_{k, free}) ,
\end{aligned}
\end{equation}
%
or more succinctly,
%
\begin{equation}
\label{eq:sigmoid_inv_obs_model_free}
p(m[j] \mid \bfx_t, z_t[k]) = \sigma(m[j]\theta_{k, free}). 
\end{equation}\TW{Intuitively $\theta_{occ} > 0$ and $\theta_{free} < 0$.}
%

\textit{Case 2:} $|z_t[k] - d(\bfx_t, m[j])| < \epsilon$.
One simple paramterization is to use a sigmoid function if the observation
$z_t[k]$ is close to distance $d(\bfx_t, m[j])$ by a threshold $\epsilon$.
That is, if $|z_t[k] - d(\bfx_t, m[j])| \leq \epsilon$ for some constant $\epsilon$,
\begin{equation}
\begin{aligned}
p(m[j] = 1 \mid \bfx_t, z_t[k]) &= \sigma(\theta_{k, occ}) \\
p(m[j] = -1 \mid \bfx_t, z_t[k]) &= 1 - \sigma(\theta_{k, occ}) 
\end{aligned}
\end{equation}
or more succinctly,
\begin{equation}
\label{eq:sigmoid_inv_obs_model_occ}
p(m[j] \mid \bfx_t, z_t[k]) = \sigma(m[j]\theta_{k, occ}).
\end{equation}

\textit{Case 3:} $z_t[k] < d(\bfx_t, m[j]) - \epsilon$. In this case, the
laser-scan does not provide any information about the occupancy of the cell,
i.e. the $z_t[k]$ is independent of $m[j]$. Hence, the log-odds in this case is
zero and does not contribute to the Eqn~\eqref{eq:simplified_log_odds}.

==> tex/old/Approach_2_Planning.tex <==
\section{Differentiable Planning}
\label{sec:diff_plan}

In this section, we solve the planning problem described in Eqn~\eqref{eqn:Q}
such that output policy $\pi_t$ is differentiable with respect to the cost function
$c_t$.
Value Iteration Networks (VIN)~\cite{Tamar_VIN16} shows that $T$ iterations of
the value iteration algorithm can be approximated by a neural network with $T$
convolutional and maxpooling layers.
This allows VIN to be differentiable with respect to the stage cost.
However, VIN scales poorly with environment size, since VIN performs Bellman
backups (convolutions and min-pooling) over the entire state space.
%The depth of the VIN network scales linearly with the size of the environment.
Moreover, solving for a global policy is redundant in unexplored regions of a partially observable environment.
To address these limitations, we propose a differentiable A* algorithm to
generate a local control policy at the current state.
Similar to the advantages of A* planning algorithm over Dijkstra---assuming good
heuristic---our algorithm improves the efficiency of VIN by reducing the
effective branching factor~\cite[p 103]{russell2016artificial}.
While we develop our differentiable A* algorithm to
solve the aforementioned navigation problems, the
conclusions of this section can hold for other planning algorithms
which solve Deterministic Shortest Path (DSP), e.g. dynamic programming.


%%======================= A* ===========================%

\begin{algorithm}[t]
\caption{Differentiable A* Planning Algorithm}
\label{alg:A*}
\begin{algorithmic}[1]
\State {\bfseries Input:} Current state $\bfx_t$, goal state $\bfx_g$, cost function $c_t$, heuristic $h$, heuristic weight $\epsilon$, motion model $f$
\State $g(\bfx_g) = 0, \; g(\bfx) = \infty, \; \forall \bfx \in \calX$
\State OPEN $\gets \{\bfx_g\}$, CLOSED $\gets \{\}$, PARENT$[\bfx_g] \gets null$
\While {$\bfx_t \not\in $ CLOSED}
    \State Remove $\bfx$ with smallest $g(\bfx)+\epsilon h(\bfx)$ value from OPEN and insert $\bfx$ in CLOSED
    \For {each predecessor $\bfy$ s.t. $f(\bfy, \bfu) = \bfx$ for some $\bfu$}\label{alg:predecessor}
        \If {$c_t(\bfy, \bfu) + g(\bfx) < g(\bfy)$}\label{alg:conv_min1}
            \State $g(\bfy) \gets c_t(\bfy, \bfu) + g(\bfx)$ \label{alg:conv_min2}
            \State PARENT[$\bfy$] $\gets \bfx$\label{alg:conv_min3}
        \EndIf
    \EndFor
\EndWhile
\State $Q_t(\bfx_t, \bfu_t) \gets c_t(\bfx_t, \bfu_t) + g(f(\bfx_t, \bfu_t))\; \forall \bfu_t \in \calU$ \label{alg:Q}
\Function{Derivative}{$\bfx_t, \bfu_t$, PARENT}
    \State Compute trajectory $\bftau_{(\bfx_t, \bfu_t)}$ by traversing the linked list PARENT from $f(\bfx_t, \bfu_t)$ to $\bfx_g$ \label{alg:tau}
    \State {\bfseries return} $\bfM_{(\bfx_t, \bfu_t)}$ from $\bftau_{(\bfx_t, \bfu_t)}$ by Eqn~\eqref{eqn:M}
\EndFunction
\State {\bfseries Output:} policy $\pi_t(\bfu_t \mid \bfx_t) = \frac{\exp\prl{-Q_t(\bfx_t, \bfu_t)}}{\sum_{\bfu\in \calU}\exp\prl{-Q_t(\bfx_t, \bfu)}}$, visitation matrix $\bfM_{(\bfx_t, \bfu_t)}$ = DERIVATIVE($\bfx_t, \bfu_t$, PARENT) for $\bfu_t \in \calU$
\end{algorithmic}
\end{algorithm}

Our differentiable A* algorithm which solves DSP in Eqn~\eqref{eqn:Q} and
provides derivatives with respect to the cost function is summarized in
Alg~\ref{alg:A*}.
Given the cost function $c_t$, the algorithm starts the search from the goal
state $\bfx_g$ and looks for predecessors of the motion model $f$
(line~\ref{alg:predecessor}) until it reaches the current state $\bfx_t$.
It performs convolution and min-pooling (line~\ref{alg:conv_min1}-\ref{alg:conv_min3}) only over a subset of promising states (CLOSED list) and at termination, $g(\bfx)$ will provide an upper bound to the optimal cost-to-go $V^*(\bfx)$,
%
\begin{equation}
\label{eqn:overestimate}
\begin{aligned}
g(\bfx) &= V^*(\bfx) \; &\forall \bfx &\in \text{CLOSED} \\
g(\bfx) &\geq V^*(\bfx) \; &\forall \bfx &\not\in \text{CLOSED} \;,
\end{aligned}
\end{equation}
%
where $V^*(\bfx)$ is defined as the optimal cost-to-go,
%
\begin{equation}
\begin{aligned}
& V^*(\bfx) =  \min_{\bfu_{1:T-1}}  \sum_{k=1}^{T-1} c_t(\bfx_k, \bfu_k) \\
& \text{s.t.}\;\; \bfx_{k+1} = f(\bfx_k, \bfu_k),\; \bfx_1 = \bfx,\; \bfx_T = \bfx_g.
\end{aligned}
\end{equation}
%
Therefore, $Q_t(\bfx_t, \bfu_t)$ in line~\ref{alg:Q} will be optimal, $Q_t(\bfx_t,
\bfu_t) = Q_t^*(\bfx_t, \bfu_t)$, if the successor state $f(\bfx_t, \bfu_t)$ is
in CLOSED, while it will be overestimated, and in turn the policy $\pi_t$
underestimated, for $f(\bfx_t, \bfu_t)$ not in CLOSED.
This is a desirable behavior to make the policy greedy. 

\subsection{Closed form back-propagation}
\label{sec:closed-form-back-propagation}
Not only is the Differentiable A* algorithm more efficient than dynamic
programming in forward computation of $V^*(\bfx)$,
but also it is more efficient in computing gradients.
We compute the gradients, without back-propagating through multiple convolutional and min-pooling layers.
We compute the closed form derivative of $Q_t(\bfx_t, \bfu_t)$ with respect to
the cost function $c_t$ has simple form that can be obtained directly from the
forward pass.

Let $\bftau_{(\bfx_t, \bfu_t)}$ be a sequence of state-control pairs that starts
with $(\bfx_t, \bfu_t)$, ends at $\bfx_g$ and follows the motion model
$\bfx_{k+1} = f(\bfx_k, \bfu_k)$.
Define $\bfM_{(\bfx_t, \bfu_t)}$ as the state-control visitation matrix of size $|\mathcal{X}|\times|\mathcal{U}|$ for such $\bftau_{(\bfx_t, \bfu_t)}$, where the entries are given by
\begin{equation}
\label{eqn:M}
\bfM_{(\bfx_t, \bfu_t)}[\bfx, \bfu] = 
\begin{cases}
1, \text{ if } \prl{\bfx, \bfu} \in \bftau_{(\bfx_t, \bfu_t)} \\
0, \text{ otherwise.}
\end{cases}
\end{equation}
We can then rewrite Eqn~\eqref{eqn:Q} as
\begin{equation}
\label{eqn:Q_cM}
Q^*_t(\bfx_t, \bfu_t) = \min_{\bfM_{(\bfx_t, \bfu_t)}} \langle c_t, \bfM_{(\bfx_t, \bfu_t)} \rangle_{\bfF}
% = \langle c_t, \bfM_{(\bfx_t, \bfu_t)}^* \rangle_{\bfF}
\end{equation}
\VD{Not sure if the second equality was true.}
where $\langle\cdot, \cdot\rangle_{\bfF}$ is the Frobenius inner product operator. % and $\bfM_{(\bfx_t, \bfu_t)}^*$ is the visitation matrix for optimal trajectory.
Eqn~\eqref{eqn:Q_cM} shows that the optimal $Q^*$ function can be separated into the 
cost function part and trajectory part.
The minimization only affects the cost function but not the trajectory.
We apply the subgradient method~\cite{Shor_Subgradient12} which is also used in~\cite{Ratliff_06}.
%
\begin{lemma}[Derivative at minima]
\label{lemma:subgradient}
For a differentiable function $f(\cdot, y)$, and a piece-wise convex function
$g(x) \defeq \min_y f(x,y)$,
the subgradient of the minima of the function $\partial_x g(x)$ contains the gradient
of the function $\nabla_x f(x, y^*)$ at the optimal value, where $y^* = \argmin_y f(x,y)$.
\end{lemma}
%
Applying Lemma~\ref{lemma:subgradient} to $Q^*_t(\bfx_t,\bfu_t)$, we get that the subgradient of the optimal state-control values with respect to the cost function is just the state-control visitation,
%
\begin{equation}
    \frac{\partial Q^*_t(\bfx_t,\bfu_t)}{\partial c_t} = \bfM^*_{(\bfx_t, \bfu_t)} \;,
\end{equation}
%
which can be obtained by traversing through the linked list PARENT in
line~\ref{alg:tau}. In summary, our differentiable A* algorithm is efficient to
perform convolutions only on a subset of the state space and is differentiable
with respect to the parameterization $\bftheta$ of the cost function $c_t$.
These properties make the algorithm significantly more scalable with respect to
the size of the state space.
\VD{I am not sure if $\bfM^*_{(\bfx_t, \bfu_t)}$ is independent of $c_t$}.






















%In this section, we will develop planning algorithms over the learned cost function $\hat{c}_t^{\theta}$ while ensuring that the output stochastic policy $\pi_t^{\theta}$ is differentiable with respect to $\hat{c}_t^{\theta}$. Value iteration networks (VIN)~\cite{Tamar_VIN16} has shown that the value iteration algorithm can be approximated by a neural net architecture with convolutional and maxpooling layers. While VIN makes the planning model differentiable and allows backpropagation, we argue that convolutional operations over the entire state space are computationally expensive and do not scale with the size of the state space and the planning horizon. As a solution to this issue, we first propose a differentiable dynamic programming model, inspired by VIN, that solves the deterministic shortest path problem on $\hat{c}_t^{\theta}$. We then propose a differentiable A* algorithm that only performs local convolutional operations that encode Bellman backups on a subset of promising states.



%\subsection{Differentiable Dynamic Programming}
%\label{sec:diff_dp}
%The original VI module in VIN solves the infinite horizon stochastic shortest path problem. Inspired by the VI module, we propose a differentiable dynamic programming (DP) algorithm that solves the finite-horizon deterministic shortest path problem as follows. Let $V(x)$ be the optimal cost-to-go from each state $x$ to $x_g$, with respect to the cost function $\hat{c}_t^{\theta}$,
%\begin{equation}
%\begin{aligned}
%& V(x) =  \min_{u_{1:T-1}}  \sum_{\tau=1}^{T-1} \hat{c}_t^{\theta}(x_{\tau}, u_{\tau}) \\
%& \text{s.t.}\;\; x_{\tau+1} = f(x_{\tau}, u_{\tau}),\; x_1 = x,\; x_T = x_g.
%\end{aligned}
%\end{equation}
%The optimal cost-to-go $V(x)$ for all states $x$ can be obtained at the last step of the differentiable DP algorithm (Algorithm~\ref{alg:1}). To enforce differentiability, we implement the Bellman equations in line 10 and 11 of Algorithm~\ref{alg:1} with neural net layers as inspired by VIN. We implement $V(x)$ as a vector of size $|\mathcal{X}|$ and $Q(x,u)$ as a matrix of size $|\mathcal{X}|\times|\mathcal{U}|$. Let $\delta(x) \in \crl{0,1}^{|\mathcal{X}|}$ be a kronecker delta function
%\begin{equation}
%\begin{aligned}
%    \delta(x) = 
%    \begin{cases}
%    1, \text{ if } x = 0, \\
%    0, \text{ otherwise.}
%    \end{cases}
%\end{aligned}
%\end{equation}
%The optimal cost-to-go at the next state $V(f(x_{\tau}, u_{\tau}))$ can be obtained by having a convolutional layer on $V(x)$ with $\delta(f(x_{\tau}, u_{\tau})-x)$ as the convolutional kernel that accounts for the deterministic transitions from $x_{\tau}$ to $f(x_{\tau}, u_{\tau})$,
%\begin{equation}
%\begin{aligned}
%V(f(x_{\tau}, u_{\tau})) &= \sum_{s=0}^{|\mathcal{X}-1|} \delta(f(x_{\tau}, u_{\tau})-s) V(s) 
%\end{aligned}
%\end{equation}
% The quantity $Q(x_{\tau}, u_{\tau})$ is then min-pooled along the control channel to get $V(x_{\tau})$ for the next iteration. \TW{This does not look like the algorithmic environment and I cannot use the Return command in function.}
% 
%\begin{algorithm}[t]
%\caption{Differentiable Dynamic Programming}
%\label{alg:1}
%\begin{algorithmic}[1]
%\STATE {\bfseries Input:} Current state $x_t$, goal state $x_g$, cost function $\hat{c}_t^{\theta}$, deterministic transition $f$
%\FUNCTION{Conv($V(x), \delta({f(x_{\tau},u_{\tau})} - x) $)}
%    \STATE {\bfseries return} $\sum_{s=0}^{|\mathcal{X}-1|} \delta(f(x_{\tau}, u_{\tau})-s) V(s) $
%\ENDFUNCTION

%\FUNCTION{Minpool($Q(x_{\tau},u_{\tau})$)}
%    \STATE {\bfseries return} $\min_{u_{\tau} \in \mathcal{U}} \crl{Q(x_{\tau}, u_{\tau})}$
%\ENDFUNCTION

%\STATE $V(x_g) \leftarrow 0$, $V(x) \leftarrow \infty \; \forall x \in \mathcal{X} \setminus x_g$

%\FOR{$\tau = T-1:1$}
%    \STATE $Q(x_{\tau}, u_{\tau}) \leftarrow \hat{c}_t^{\theta}(x_{\tau}, u_{\tau}) + \text{Conv}(V(x), \delta({f(x_{\tau},u_{\tau})} - x)), \; \forall x_{\tau} \in \mathcal{X} \setminus x_g$ and  $\forall u_{\tau} \in \mathcal{U}$
%    \STATE $V(x_{\tau}) \leftarrow \text{Minpool }( Q(x_{\tau}, u_{\tau})), \; \forall x_{\tau} \in \mathcal{X} \setminus x_g$ 
%\ENDFOR
%\STATE {\bfseries Output:} Policy $\pi_t^{\theta}(u_t|x_t) = \frac{\exp{\big(-Q(x_t, u_t)\big)}}{\sum_{u_t'\in \mathcal{U}}\exp{\big(-Q(x_t, u_t')\big)}}$ 
%\end{algorithmic}
%\end{algorithm}


%The differentiable DP algorithm is a straightforward extension of the VI module in VIN with deterministic transitions and finite planning horizon by having kronecker delta convolutional kernels and clamping $V(x_g) = 0 $ throughout the iterations. Both the VI module and the differentiable DP algorithm output differentiable policy by using neural net layers and require convolutional operation over the entire state space. However, differentiable DP is guaranteed to converge in iterations that are at most the length of the planning horizon while the VI module has to terminate in some fixed iterations to approximate the value iteration algorithm.



%\subsection{Differentiable A* Planning}
%\label{sec:diff_A}
%Next, we present the more computationally efficient planning algorithm, differentiable A* algorithm, which does not have convolutional layers over the entire state space but only consider local convolutions over a subset of promising states. The key observation is that we can replace the optimal cost-to-go $V(x)$ from $x$ to $x_g$ in the differential dynamic programming algorithm with the $g$-values obtained from A* algorithm. Assuming that the cost of an optimal path from any state $x$ to any other state $x'$ is the same as that from $x'$ to $x$, we initialize A* from $x_g$ and search for the optimal path from the goal state $x_g$ to the current state $x_t$. When Algorithm~\ref{alg:2} terminates, $g(x)$ forms an upper bound for $V(x)$,
%\begin{equation}
%\begin{aligned}
%g(x) = V(x) \; \forall x \in \text{CLOSED} \\
%g(x) \geq V(x) \; \forall x \not\in \text{CLOSED}.
%\end{aligned}
%\end{equation}
%The differentiability is again guaranteed in line 9 and 10 by implementing $g(f(x_{\tau},u_{\tau}))$ as the convolution of $g(x)$ with kronecker delta kernels $\delta(f(x_{\tau},u_{\tau})-x)$ accounting for the deterministic transitions from $x_{\tau}$ to $f(x_{\tau},u_{\tau})$ and min-pooling between the quantities $g(f(x_{\tau},u_{\tau}))$ and $ \hat{c}_t^{\theta}(x_{\tau},u_{\tau}) + g(x_{\tau})$. The convolutional operator is not applied to the entire state space but only locally on states popped from the OPEN list. Not only is differentiable A* algorithm more efficient than dynamic programming in obtaining the optimal cost-to-go $V(x_t)$ in the forward computation, it is also more efficient in constructing a correct gradient without backpropagating through multiple layers of convolutional and minpooling layers in the dynamic programming algorithm. The derivative of the $g$-values with respect to the cost function $\hat{c}^{\theta}_t$ has simple form as shown in Prop.~\ref{prop:1} and the proof is given in Appendix~\ref{app:a}. This property makes differentiable A* algorithm scale with the size of the environment. It is worth pointing out that if we start from some state $x_t \in$ CLOSED, the policy will give a small probability for $u_t$ if it leads to a next state outside CLOSED because $Q(x_t, u_t)$ is overestimated for such $(x_t, u_t)$, resulting in a ``safe'' planning trajectory that is unlikely to leave the CLOSED states.


%\begin{algorithm}[t]
%\caption{Differentiable A* Planning}
%\label{alg:2}
%\begin{algorithmic}[1]
%\STATE {\bfseries Input:} Current state $x_t$, goal state $x_g$, cost function $\hat{c}_t^{\theta}$, heuristic function $h$, deterministic transition $f$
%\FUNCTION{Conv($g(x), \delta({f(x_{\tau},u_{\tau})} - x) $)}
%    \STATE {\bfseries return} $\sum_{s=0}^{|\mathcal{X}-1|} \delta(f(x_{\tau}, u_{\tau})-s) g(s) $
%\ENDFUNCTION
%\STATE $g(x_g) = 0, \; g(x) = \infty \; \forall x \in \mathcal{X}$
%\STATE OPEN $\gets \{x_g\}$, CLOSED $\gets \{\}$
%\WHILE{$x_t \not\in $ CLOSED}
%    \STATE Remove $x_{\tau}$ with smallest $f(x_{\tau}) = g(x_{\tau})+h(x_{\tau})$ from OPEN and insert $x_{\tau}$ in CLOSED
%    \STATE $g(f(x_{\tau}, u_{\tau})) \gets \text{Conv}(g(x), \delta({f(x_{\tau},u_{\tau})} - x)), \; \forall u_{\tau} \in \mathcal{U}$
%    \STATE $g(f(x_{\tau}, u_{\tau})) \gets \min\{g(f(x_{\tau}, u_{\tau})), \hat{c}_t^{\theta}(x_{\tau},u_{\tau}) + g(x_{\tau})\}, \; \forall u_{\tau}\in \mathcal{U}$ 
%\ENDWHILE
%\STATE $Q(x_t, u_t) \gets \hat{c}_t^{\theta}(x_t, u_t) + g(f(x_t, u_t))\; \forall u_t \in \mathcal{U}$
%\STATE {\bfseries Output:} Policy $\pi_t^{\theta}(u_t|x_t) = \frac{\exp{\big(-Q(x_t, u_t)\big)}}{\sum_{u_t'\in \mathcal{U}}\exp{\big(-Q(x_t, u_t')\big)}}$
%\end{algorithmic}
%\end{algorithm}



%\begin{proposition}
%\label{prop:1}
%For any current state $x_t \in \mathcal{X}$, let $g(x_t)$ be the cost of an optimal path from $x_t$ to the goal state $x_g \in \mathcal{X}$ as obtained in Alg.~\ref{alg:2}. We further assume that such optimal path is unique. Given any state $x \in \mathcal{X}$ and control $u \in \mathcal{U}$, the derivative $\frac{\partial g(x_t)}{\partial \hat{c}_t^{\theta}(x, u)}$ can be obtained as follows,
%\begin{equation}
%    \frac{\partial g(x_t)}{\partial \hat{c}_t^{\theta}(x, u)} = 
%    \begin{cases}
%        1, \text{ if } \hat{c}_t^{\theta}(x, u) \text{ is on the optimal path, } \\
%        0, \text{ otherwise.}
%    \end{cases}
%\end{equation}
%This derivative is the same as $\frac{\partial V(x_t)}{\partial \hat{c}_t^{\theta}(x, u)}$ by backpropagating through the differentiable dynamic programming algorithm.
%\end{proposition}





==> tex/old/Approach_3_CostAndPlanning.tex <==
\section{Cost Learning via Differentiable Planning}
\label{sec:cost_learning_planning}

Given demonstrations $\mathcal{D}$, the parameters $\bftheta$ are optimized by minimizing the cross-entropy loss $\mathcal{L}(\bftheta)$ defined in Problem~\ref{pb:1}. The computation graph in Fig.~\ref{fig:approach} is composed of a cost representation layer and a differentiable planning algorithm. Policy evaluation is differentiable end-to-end with respect to $\bftheta$ and stochastic gradient descent can be applied. For each sample $(\bfx_{1:t}, \bfu^*_t, \bfz_{1:t}, \bfx_g) \in \mathcal{D}$, the gradient of the loss ($-\log \pi_t (\bfu^*_t|\bfx_t)$) with respect to the parameters $\bftheta$ can be obtained by applying chain rule,
\begin{equation}
\begin{aligned}
\label{eq:chain_rule}
&\frac{\partial (-\log \pi_t (\bfu^*_t|\bfx_t))}{\partial \bftheta} =  \frac{(-\log \pi_t (\bfu^*_t|\bfx_t))}{\partial Q_t} \frac{\partial Q_t}{\partial c_t} \frac{\partial c_t}{\partial \bftheta} \\
&= \sum_{\bfu_t\in \mathcal{U}} \prl{\mathbbm{1}_{\{\bfu_t=\bfu^*_t\}} - \pi_t(\bfu_t|\bfx_t)}\bfM^*_{(\bfx_t, \bfu_t)} \frac{\partial c_t}{\partial \bftheta}
\end{aligned}
\end{equation}

Although the form of the gradient in Eqn~\eqref{eq:chain_rule} is similar to that in
Ziebart et al.~\cite{Ziebart_MaxEnt08}, our contributions are orthogonal.
Our contribution is to use differentiable A* which improves the
efficiency of planning that scales with the state space and provides a subgradient
to learn the cost function in backpropagation.
On the other hand, the contribution of Ziebart et al.~\cite{Ziebart_MaxEnt08} is to
use $\softmin$ instead of $\min$ in their Bellman update which results
in fair exploration of routes with high branching factor. Ziebart et
al. also maximize entropy of the policy while following the expert's demonstrations.
Both of these contributions can be included our framework, however they are not
the focus of our work and benefits of our approach can be shown without including
either. We leave the extension of our work to include the maximum entropy formulation from Ziebart et al. as future work.

Full algorithms for the training and testing phases (Fig.~\ref{fig:approach}) are shown in Alg.~\ref{alg:train} and Alg.~\ref{alg:test}.


\begin{algorithm}[h]
\caption{Training: learn cost function parameters $\theta$}
\label{alg:train}
\begin{algorithmic}[1]
\State {\bfseries Input:} Demonstrations $\mathcal{D} \!=\! \crl{(\bfx_{t,n},\bfu_{t,n}^*,\bfz_{t,n}, \bfx_{g,n})}_{t=1, n=1}^{T_n,N}\!\!$
\While{$\bftheta$ not converged}
\State $\mathcal{L}(\bftheta) \gets 0$
\For{$n = 1:N$} 
    \For{$t = 1:T$}
        \State Estimate cost function $c_{t,n}$ from current trajectory $\bfx_{1:t, n}$ and observation history $\bfz_{1:t, n}$ as in Sec.~\ref{sec:cost_rep}.
        \State Obtain stochastic policy $\pi_{t,n}$ from $c_{t,n}$ as in Sec.~\ref{sec:diff_plan}.
        \State $\mathcal{L}(\bftheta) \gets \mathcal{L}(\bftheta) -\log \pi_{t, n} (\bfu_{t,n}^*|\bfx_{t,n})$ 
    \EndFor
\EndFor
\State $\bftheta \gets \bftheta - \alpha \nabla \mathcal{L}(\bftheta)$ obtained via Eq.~\eqref{eq:chain_rule}
\EndWhile
\State {\bfseries Output:} $\bftheta$ 
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
\caption{Testing: compute control policy for learned $\bftheta$}
\label{alg:test}
\begin{algorithmic}[1]
\State {\bfseries Input:} Start state $\bfx_s$, goal state $\bfx_g$, optimized $\bftheta$ 
\State Current state $\bfx_t \gets \bfx_s$
\While{$\bfx_t \neq \bfx_g$}
    \State Make an observation $\bfz_t$
    \State Estimate cost function $c_t$ from current trajectory $\bfx_{1:t}$ and observation history $\bfz_{1:t}$ as in Sec.~\ref{sec:cost_rep}.
    \State Obtain stochastic policy $\pi_t$ from $c_t$ as in Sec.~\ref{sec:diff_plan}
    \State Execute a control $\bfu_t$ from policy $\pi_t(\cdot|\bfx_t)$ and transition to the next state $\bfx_{t} \gets f(\bfx_t, \bfu_t)$
\EndWhile
\State {\bfseries Output:} Navigation succeeds or fails.
\end{algorithmic}
\end{algorithm}



==> tex/old/DiscardedSnippets.tex <==
% From: tex/Introduction.tex
% X (+define X if not obvious) is an important problem
%% VD: I don't think you need these lines.
% Safe navigation is an important problem for robotic systems in transportation
% and delivery.
% Practical applications of autonomous robot systems increasingly require
% operation in unstructured, partially known, and dynamically changing
% environments.
% Achieving safe and robust navigation in such conditions is directly coupled with
% the quality of the environment representation and the cost function design.
% In a motion planning problem, a robot is required to search for a sequence of decisions or controls that achieves a pre-defined goal, while taking the environment structure and robot dynamics into account.
%The robot has to take into account both its own dynamics and those of the environment in order to produce a collision-free and feasible trajectory.

% The core challenges are this and that.
%\textcolor{red}{This version on map representation is not strong, should use cost instead}One core challenge in path planning is that the map representation is not designed for the planning problem. Mapping is considered as a separate topic that aims at constructing a complete and accurate representation of the environment from sensory data. It ignores the fact that a lot of information is irrelevant for the planning problem. In contrast, humans and animals are able to filter out obstacle information if it does not interfere with the planning task and adapt from previous planning experience when a new obstacle configuration is encountered. This observation motivates the design of a model that can learn from experience a map representation that is effective for the planning problem. Specifically, the model should have a map representation that can be optimized by the planning algorithm so that it only contains planning-relevant information. In addition, the map representation should be able to adapt to observed obstacles in a partially observable environment. 


% 2. Even environment representation is hard to define. Especially it's resolution.
However, not much work has been done on the similar limitations in context of
efficient environment or latest space representation.
A typical approach in autonomous driving, such as Probabilistic occupancy
mapping~\cite{Hornung_Octomap13,voxblox}, is to construct highly detailed
maps of the city that even include irrelevant details like 3D shape of the tree.
In contrast, humans and animals are able to filter out obstacle information that
does not interfere with the navigation task and adapt based on prior planning
experience when new obstacle configurations are encountered.

% In this work we do W (?).
%Our main contribution is a semi-parametric mapping and planning (SPMP) model for a robot that navigates in a partially observable environment. SPMP uses a parametric latent map representation that can be used for and optimized by planning algorithms. The latent map representation can be cascaded, in principle, with any non-parametric path planning algorithm as long as the planner policy is differentiable with respect to the parameters of latent map. The novelty of our approach is that we make the SPMP model fully differentiable so that the planner performance can be used to optimize the latent map representation using standard gradient descent. Hence, the latent map is learned to capture the salient features in the environment that allow the planner to achieve a good performance in a navigation task. As shown in the experiments, learning such navigation-specific latent maps can help differentiate between important obstacles that may be along the optimal path and trivial obstacles that the planner does need to be aware of while still accomplishing the task.

More recently, Value Iteration Networks (VIN)~\cite{Tamar_VIN16} were proposed
that address the challenge of learning cost functions and maps by directly
back-propagating the loss to the map representation.
However, VINs operate the full environment state at all times and hence their depth scale poorly with environment size.
VINs solve for a global policy, which is redundant in unexplored regions of a
partially observable environment.


% Experiment tables
\begin{table*}[t]
    \centering
    \begin{tabular}{|| c | c |  c | c | c | c | c | c | c | c ||}
        \hline
        Model & Cost encoder & \makecell{Train \\ loss} & \makecell{Train acc.} & \makecell{Val. \\ loss} & \makecell{Val. acc.} & \makecell{Test \\ succ. rate} & \makecell{Test \\ traj. diff.} & \makecell{Test traj \\ too long} & Hit obstacle   \\
        \hline
        Deep MaxEnt & CNN & $0.14$ & $94.8\%$ & $0.18$  & $93.6\%$ & $866/952$ & $0.145$ & $3/952$ & $83/952$  \\
        \hline
        Ours & $s=1, l=100$ & $1.11$ & $59.2\%$ & $1.10 $  & $59.5\%$ & $950/952$ & $0.378$ & $0/952$ & $2/952$  \\
        \hline
        Ours & \makecell{learnable \\ $s=4.6, l=9.6$} & $0.65$ & $62.3\%$ & $0.66$  & $62.1\%$ & $926/952$ & $0.174$ & $0/952$ & $26/952$  \\
        \hline
        Ours & CNN & $0.25$ & $91.2\%$ & $0.27$  & $90.5\%$ & $921/952$ & $0.144$ & $0/952$ & $31/952$  \\
        \hline

    \end{tabular}
    \caption{Training and test results in $16\times16$ gridworld domain}
    \label{tb:map16_results}
\end{table*}


\begin{table*}[t]
    \centering
    \begin{tabular}{|| c | c |  c | c | c | c | c | c | c | c ||}
        \hline
        Model & Cost from map & \makecell{Train \\ loss} & \makecell{Train acc.} & \makecell{Val. \\ loss} & \makecell{Val. acc.} & \makecell{Test \\ succ. rate} & \makecell{Test \\ traj. diff.} & \makecell{Test traj \\ too long} & Hit obstacle   \\
        \hline
        Deep MaxEnt & N/A & $0.06$ & $97.5\%$ & $0.23$  & $93.7\%$ & $38/122$ & $6.528$ & $11/122$ & $73/122$  \\
        \hline
        Ours & $s=1, l=100$ & $1.34$ & $39.5\%$ & $1.32 $  & $42.2\%$ & $122/122$ & $2.876$ & $0/122$ & $0/122$  \\
        \hline
        Ours & \makecell{learnable \\ $s=5.1, l=15.4$} & $0.65$ & $62.3\%$ & $0.66$  & $62.1\%$ & $103/122$ & $1.569$ & $0/122$ & $19/122$  \\
        \hline
        Ours & CNN & $0.09$ & $96.9\%$ & $0.14$  & $95.1\%$ & $110/122$ & $1.196$ & $0/122$ & $12/122$  \\
        \hline

    \end{tabular}
    \caption{Training and test results in $100\times100$ gridworld domain}
    \label{tb:map100_results}
\end{table*}

\begin{table*}[t]
    \centering
    \begin{tabular}{|| c |  c | c | c | c | c | c | c | c ||}
        \hline
         Noise std. & \makecell{Train \\ loss} & \makecell{Train acc.} & \makecell{Val. \\ loss} & \makecell{Val. acc.} & \makecell{Test \\ succ. rate} & \makecell{Test \\ traj. diff.} & \makecell{Test traj \\ too long} & Hit obstacle   \\
        \hline
        0.05 & $0.25$ & $91.2\%$ & $0.27$  & $90.5\%$ & $921/952$ & $0.144$ & $0/952$ & $31/952$  \\
        \hline
        0.1 & $0.23$ & $92.1\%$ & $0.27$  & $91.4\%$ & $935/964$ & $0.165$ & $0/952$ & $29/964$  \\
        \hline
        0.2 & $0.34$ & $88.6\%$ & $0.34$  & $88.4\%$ & $860/937$ & $0.188$ & $0/952$ & $77/952$  \\
        \hline
        0.5 & $0.27$ & $90.4\%$ & $0.28$  & $90.1\%$ & $846/953$ & $0.129$ & $0/952$ & $107/953$  \\
        \hline

    \end{tabular}
    \caption{Training and test results of Ours in $16\times16$ gridworld domain with respect to noise}
    \label{tb:map16_noise}
\end{table*}


Experiments > Dataset > Details
We randomly generate $7638$ and $970$ maps in the two map size domains and sample 
10 trajectories on each map.
The trajectories are obtained by running an optimal planning algorithm to solve the 
determistic shortest path problem on the fully observable map.
This results in $514k$ and $460k$ samples of the form $(\bfx_{1:t}, \bfu_t^*, \bfz_{1:t}, \bfx_g)$ 
in the training set $\mathcal{D} = \crl{(\bfx_{t,n},\bfu_{t,n}^*,\bfz_{t,n}, \bfx_{g,n})}_{t=1, n=1}^{T_n, N}$ 
for the two domains. 
The validation and test sets are prepared similarly on another $966$ and $122$ maps, resulting in 
$66k$ and $58k$ samples in the two domains respectively.  

In testing, we randomly generate another $952$ and $122$ maps with one start and goal 
location for each map. 
The robot iteratively processes the new observation $\bfz_t$ to get the cost function 
$c_t$ and takes the greedy action $\bfu_t = \argmax \pi_t(\cdot \mid \bfx_t)$ to get 
to the next state. 

==> tex/old/Introduction-with-related-work-weaved-in.tex <==
\section{Introduction}
\label{sec:introduction}
%\VD{Let's use a git-friendly convention to wrap lines. Let's us keep no more than one sentence per line. A sentence can span several lines, but not vice-versa. This helps in git-diff and git-merge operations.}
%% Write an outline first. Each paragraph should convey one point of the
%% argument. A typical outline of introduction.
% 1. Q: Start with the broadest base, a well accepted problem or technique
% 2. Q: What are the typical/SOTA ways of solving that problem.
% 3. Q: What are the limitations of SOTA ways solving problem
% 4. Q: What do you propose
% 5. Q: How does it solve the problem
% 6. Q: Tell me more . Where can I find more information. Refer to sections, to
% allow a familiar reader to jump to the different sections.
% 7. Q: What are your novel contributions

%% This paper outline
% 1. Setup the problem and that we are going to solve it by IRL
% 2. Give more details of the problem. Why is this problem important?
% 3. What do we propose? Efficient rollout of states (ERoS) and closed form %
%    gradient (CfG) computation.
% 4. There a few works that address IRL in POE, but we are more efficient with
%    ERoS and CfG.
% 4. Contributions.


% 1. No one does both, but we will
Consider the problem of a robot navigating to a goal in an unknown environment.
To address this problem we need to either design a cost function or learn the cost function from expert demonstrations.
We focus on the latter approach, because the \textit{true} cost function requiring safe, dynamically feasible, and efficient behavior, is typically not known and hard to design.
The field of Inverse Reinforcement Learning (IRL) deals with learning cost function from demonstrations.

In this work, we focus on learning the navigation costs in partially observable environments.
Given expert demonstrations of robot navigating to goals we want to learn a policy
that imitates the expert as closely as possible.
We assume that the demonstration information includes trajectories of
expert pose, control, observation and desired goals.
The robot pose and robot model are assumed to be known but the cost function and
map of the environment are not known.
Many practical tasks can be formulated as this problem, for example, an
autonomous car tasked with going to a particular latitude-longitude through an
unknown environment.

Several works have addressed similar but not exactly the same problem.
Choi~and~Kim~\cite{ChoiIRLinPOMDPJMLR2011} address inverse reinforcement
learning in partially observable environments.
However they assume ``belief trajectories'' to be given as a part of the
demonstrations, while we focus on learning the map probabilities (aka belief)
representation from observations.

A series of recent works \cite{Shankar_RLviaRCNN2016, Karkus_QMDPNet2017,
Karkus_DAN19}, address robotic navigation under partial observability.
Most of these works assume that the map of the environment is known while
the robot-pose has to be estimated from partial observations.
In Karkus~\etal/~\cite{Karkus_DAN19}, the assumption is relaxed to include
only partial knowledge of the map, i.e. the structure of building is known but
the placement of furniture is not known.
This is different from the problem that we are interested in, where the
robot-pose is known but the map is fully unknown.
The approach used in these works is the formulation of robotic-navigation as a
POMDP~\cite{ASTROM_POMDP1965}, where the uncertain parts of the problem are
modeled as the state of POMDP.
If the entire map is included as part of the state, then state space is
exponential in map size and so is the complexity of used POMDP algorithms.
Instead we directly learn the cost function as the non-stationary expected value
over the current belief of the map.

%
\begin{figure}%
  %\includegraphics[width=\linewidth]{fig/PlanningAlgorithmAdvantage.pdf}
  \includegraphics[width=\linewidth]{fig/approach-with-planning-advantage.pdf}
  \caption{
   Architecture for learning cost function representations from
   demonstrations.
   Our main contribution lies in designing an efficient planning block
   that uses a motion-planning algorithm (e.g. A*, RRT etc.)
   to plan a trajectory over a subset of states.
   We also use closed-form gradient solution of the cost-to-go with respect to the
   cost function, which holds for any optimal planning algorithm.
   The figure in right-bottom shows how an A* like motion planning algorithm
   is more efficient than Value Iteration Networks.
   The A* algorithm will update cost-to-go estimates only in the promising
   subset of state space rather than the entire state space, which is
   particularly redundant in partially observable environments.}\TW{remove $\theta$ superscript in $c_t$ and $\pi_t$}%
  \label{fig:planning-advantage}%
  \label{fig:approach}
\end{figure}%
% 

Lately, Value Iteration Networks (VIN)~\cite{Tamar_VIN16}
has become the standard planning approach in learning algorithms.
Gupta~\etal/~\cite{Gupta_CMP17} proposed an approach for visual navigation in
partially observable environments. Ziebard~\etal/~\cite{Ziebart_MaxEnt08}
use maximum entropy based exploration while imitating expert demonstrations.
Both of these works use VIN.
VIN requires an update of the \textit{cost-to-go} estimates for \emph{all}
states at each iteration.
Another one of our insights is that in partially observable environments, the cost-to-go
estimates need to be updated for only a \emph{subset} of states.
These are the promising states that the motion-planning algorithm is expects to
visit on the path to the desired goal.
We show that any motion planning algorithm (e.g., A*~\cite{ARA},
RRT~\cite{Lavalle_RRT98,Karaman_RRTstar11}, etc.) that
returns the optimal cost-to-go over a promising subset of states is enough to
provide an accurate trajectory (see Fig~\ref{fig:planning-advantage}).
In particular, we implement the A* algorithm which uses a domain-dependent
heuristic function to reduce the number of states on which \textit{cost-to-go}
estimates are updated at every iteration, thus vastly improving efficiency of
dynamic programming dependent algorithms like~\cite{Ziebart_MaxEnt08,
Gupta_CMP17, Tamar_VIN16}.


% 7. And to compute gradients in closed-form.
We further improve the efficiency of our training framework by computing closed-form
gradients of \textit{cost-to-go} with respect to the learned cost function for
any optimal planning algorithm. The main idea for this closed form solution is the
same as in Ratiff~\etal/~\cite{Ratliff_06} and similar to
Ziebart~\etal/~\cite{Ziebart_MaxEnt08}.
However, Ziebart~\etal/~\cite{Ziebart_MaxEnt08} is not able to take the full advantage
of the closed-form gradient because they still have to perform dynamic
programming to compute gradient through the planning algorithms owing to
the use of stochastic policy.


In summary, we offer the following three contributions, that are differentiated from
closely related works in Table~\ref{tab:related-work}.
%\begin{itemize} % VD: Removing itemize for space.
%\item
Firstly, we propose a planning algorithm
    that updates \textit{cost-to-go} estimates 
    only on a promising subset of states, thereby increasing the efficiency of the algorithm.
    We also incorporate efficient closed-form gradient computation from
    Ratiff~\etal/~\cite{Ratliff_06} and is described in Section~\ref{sec:cost_learning}.
  %\item
    Secondly, we offer a learnable non-stationary cost function representation
    that are directly learned as expected cost over the belief space.
   %\item
   Lastly, the cost-function representation and proposed planning
     algorithm are combined in an end-to-end trainable framework. This framework
     is implemented and evaluated to show its
     accuracy and efficiency in 2D grid world and 3D CARLA simulator environment
     (see Fig.~\ref{fig:approach}).
%\end{itemize}


\begin{table}
  \centering
  \begin{tabular}{lllll}
    \toprule
    $\downarrow$Reference \textbackslash Feature $\rightarrow$ & POE & ERoS & CfG
    \\
    \midrule
    CMP~\cite{Gupta_CMP17} & \cmark & \xmark & \xmark
    \\
    MaxEntIRL~\cite{Ziebart_MaxEnt08} & \xmark & \xmark & \cmark$^*$
    \\
    MaxMarginIRL~\cite{Ratliff_06} & \xmark & \xmark & \cmark
    \\
    DAN~\cite{Karkus_DAN19} & \cmark$^\dagger$ & \xmark & \xmark
    \\
    Ours & \cmark & \cmark & \cmark
    \\
    \bottomrule
  \end{tabular}
  \caption{Comparison with closely related work. Partially Observable Environments (POE),
    Efficient Rollout of States (ERoS) and Closed-form Gradients (CfG).
    $^*$ MaxEntIRL~\cite{Ziebart_MaxEnt08} is not able to take the full advantage
   of the closed-form gradient because they still have to perform full dynamic
    programming updates to compute gradient through the planning algorithms owing to
    the use of stochastic policy.
    $^\dagger$ DAN~\cite{Karkus_DAN19} works with uncertainty only on the
    location of robot or furniture. They assume the main structure of the map is
    known.}
  \label{tab:related-work}
\end{table}


==> tex/old/Introduction.tex <==
\section{Introduction}
\label{sec:introduction}
%\VD{Let's use a git-friendly convention to wrap lines. Let's us keep no more than one sentence per line. A sentence can span several lines, but not vice-versa. This helps in git-diff and git-merge operations.}
%% Write an outline first. Each paragraph should convey one point of the
%% argument. A typical outline of introduction.
% 1. Q: Start with the broadest base, a well accepted problem or technique
% 2. Q: What are the typical/SOTA ways of solving that problem.
% 3. Q: What are the limitations of SOTA ways solving problem
% 4. Q: What do you propose
% 5. Q: How does it solve the problem
% 6. Q: Tell me more . Where can I find more information. Refer to sections, to
% allow a familiar reader to jump to the different sections.
% 7. Q: What are your novel contributions

%% This paper outline
% 1. Two challenges:
%    + IRL: Cost functions are hard to define. People focus on that often: IRL
%    + Partially observable environments are important. Very few people combine
%    IRL and POMDPs
% 2. If we apply VIN directly to POE, we get poorly scalable solutions.
% 3. What do we propose? Efficient rollout of states (ERoS) and closed form %
%    gradient (CfG) computation.
% 4. There a few works that address IRL in POE, but we are more efficient with
%    ERoS and CfG.
% 4. Contributions.


% 1. There are two challenges: IRL and POE
Two core challenges in robotic-navigation are cost function design and partial 
observability of the environment.
Regarding the first challenge, it is widely acknowledged that the \textit{true}
cost function requiring safe, dynamically feasible, and efficient behavior, is
typically not known and hard to design~\cite{Ng_IRL00}.
The field of Inverse Reinforcement Learning (IRL)~\cite{Ng_IRL00,Sutton_RL18} addresses
this by learning the cost function from expert demonstrations instead of engineering
them.
However, most works in IRL~\cite{Ziebart_MaxEnt08, Hadfield_IRD17, Ratliff_06} are
based the assumption of fully observable environment.
This assumption does not hold in most unstructured environments due to
challenges like unavailability of maps, changing environments, occlusion etc.
For the second challenge, many works learn
different parts of the navigation pipeline, e.g. robot model, map
representation and sensor model, in partially observable
environments~\cite{Tamar_VIN16, Gupta_CMP17, Khan_MACN18, Oh_ActPred15}.
However, these works assume a readily available cost function. \TW{Is this true?}

% 4. No one does both, but we will
In this work, we focus on the
crucial problem of addressing both the challenges simultaneously, i.e.
learning the cost function in partially observable
environments, while also learning the sensor model and map representation.
% 4.1. Okay, admittedly there are a few works that do focus on both the
% challenges, IRL in POE
Many works address IRL in partially observable environments.
Choi~and~Kim~\cite{ChoiIRLinPOMDPJMLR2011} assume ``belief trajectories'' to be
given as a part of the demonstrations. In contrast, we want to learn the map
(aka belief) representation as a part of the training process.
VI-RCNNs~\cite{Shankar_RLviaRCNN2016} focus on learning a model of the
environment hence it does not generalize to unseen ones.
QMDP-net~\cite{Karkus_QMDPNet2017} like many recent works~\cite{Ziebart_MaxEnt08, Gupta_CMP17}, uses Value Iteration Networks (VIN)~\cite{Tamar_VIN16} which has become 
the standard planning approach to allow differentiability for learning.
However, VIN requires an update of the \textit{cost-to-go} estimates for all states at
each iteration.
This update is particularly redundant in partially observable environments
because of lack of accurate information about unexplored states.
As a result, these algorithms scale at least quadratically in 
the size of the environment in the worst case.

%
\begin{figure}%
  \includegraphics[width=\linewidth]{fig/PlanningAlgorithmAdvantage.pdf}
  \caption{The advantage of using motion-planning algorithm (e.g. A*, RRT etc.)
    that plans a trajectory over a subset of states over dynamics programming
    based approach like Ziebart~\etal/~\cite{Ziebart_MaxEnt08}.
    An A* like motion planning algorithm will update the
    cost-to-go estimates only in the promising subset of state space while
    dynamics programming based approach will update cost-to-go estimates in the
    entire state space.}%
  \label{fig:planning-advantage}%
\end{figure}%
% 

% 6. Our solution is to have efficient rollout of the states.
To address the scalability of these algorithms, we show that any motion planning algorithm (e.g., A*~\cite{ARA},
RRT~\cite{Lavalle_RRT98,Karaman_RRTstar11}, etc.)~\VD{We need a name for this
  contribution. We might be forced to make this the primary contribution.} that
returns the optimal cost-to-go over a promising subset of states is enough to
provide an accurate trajectory (see Fig~\ref{fig:planning-advantage}).
We implement the A* algorithm which uses a domain-dependent heuristic function to reduce
the number of states on which \textit{cost-to-go} estimates are updated at every
iteration, thus vastly improving efficiency of dynamic programming dependent algorithms
like~\cite{Ziebart_MaxEnt08, Gupta_CMP17, Tamar_VIN16}.
In this regard our work is closely related to DAN~\cite{Karkus_DAN19},
which uses the SARSOP~\cite{Kurniawati_SARSOP08} algorithm. SARSOP~\cite{Kurniawati_SARSOP08}
works by expanding only the reachable set of the belief space under the optimal
policy instead of the full belief space.
However, DAN~\cite{Karkus_DAN19} works with partial or full knowledge of the map 
and uncertainty about the robot location.
Our assumption is the reverse. We assume the location of the robot to be known and
the map as unknown, which leads to a much larger belief space.

% 7. And to compute gradients in closed-form.
We further improve the efficiency of our training framework by computing closed-form
gradients of \textit{cost-to-go} with respect to the learned cost function for
any optimal planning algorithm. The main idea for this closed form solution is the
same as in Ratiff~\etal/~\cite{Ratliff_06} and similar to
Ziebart~\etal/~\cite{Ziebart_MaxEnt08}.
However, Ziebart~\etal/~\cite{Ziebart_MaxEnt08} is not able to take the full advantage
of the closed-form gradient because they still have to perform dynamic
programming to compute gradient through the planning algorithms owing to
the use of stochastic policy.

We learn a cost function that depends upon the local belief of the environment
allowing it to ignore unexplored parts of the environment. For example, in the
occupancy grid map representation, we model the cost function depend only on the
neighboring cells rather than the full belief space of the map. This allows us
to compute the expected value of the cost function analytically. 

In summary, we offer the following three contributions, which differ from
closely related works in Table~\ref{tab:related-work}.
%\begin{itemize} % VD: Removing itemize for space.
%\item
Firstly, we propose an efficient planning algorithm
    that updates \textit{cost-to-go} estimates 
    only on a promising subset of states, thereby increasing the scalability of the algorithm.
    We also incorporate efficient closed-form gradient computation from
    Ratiff~\etal/~\cite{Ratliff_06} and is described in Section~\ref{sec:cost_learning}.
  %\item
    Secondly, we offer a trainable cost function representation that works for
   partially observable environments and can be learned from expert demonstrations.
   %\item
   Lastly, the cost-function representation and proposed planning
     algorithm are combined in an end-to-end trainable framework. This framework
     is implemented and evaluated to show its
     accuracy and efficiency in 2D grid world and 3D CARLA simulator environment
     (see Fig.~\ref{fig:approach}).
%\end{itemize}


\begin{table}
  \centering
  \begin{tabular}{lllll}
    \toprule
    $\downarrow$Reference \textbackslash Feature $\rightarrow$ & IRL & POE & ERoS & CfG
    \\
    \midrule
    CMP~\cite{Gupta_CMP17} & \cmark & \cmark & \xmark & \xmark
    \\
    MaxEntIRL~\cite{Ziebart_MaxEnt08} & \cmark & \xmark & \xmark & \cmark$^*$
    \\
    MaxMarginIRL~\cite{Ratliff_06} & \cmark & \xmark & \xmark & \cmark
    \\
    VIN~\cite{Tamar_VIN16} & \cmark & \xmark & \xmark & \xmark
    \\
    QMDP-Net/~\cite{Karkus_QMDPNet2017} & \cmark & \cmark & \xmark & \xmark
    \\
    DAN~\cite{Karkus_DAN19} & \cmark & \cmark & \cmark$^+$
    \\
    Ours & \cmark & \cmark & \cmark & \cmark
    \\
    \bottomrule
  \end{tabular}
  \caption{Comparison with closely related work. The features abbreviations are: Inverse
    Reinforcement Learning (IRL), Partially Observable Environments (POE),
    Efficient Rollout of States (ERoS) and Closed-form Gradients (CfG).
    $^*$ MaxEntIRL~\cite{Ziebart_MaxEnt08} is not able to take the full advantage
   of the closed-form gradient because they still have to perform full dynamic
    programming updates to compute gradient through the planning algorithms owing to
    the use of stochastic policy.
    $^+$ DAN~\cite{Karkus_DAN19} work on a smaller belief space with uncertainty only on
   the location of robot or furniture, while we do not make any assumptions
   about the map, but we assume that the location of the robot is known.}
  \label{tab:related-work}
\end{table}


==> tex/old/Problem_old.tex <==
\section{Problem Formulation}
\label{sec:problem_formulation}
Consider a robot navigating in an unknown environment with the task of reaching a goal state $x_g \in \mathcal{X}$. Let $x_t \in \mathcal{X}$ be the robot state, capturing its pose, twist, etc., at discrete time $t$. For a given control input $u_t \in \mathcal{U}$, the robot state evolves according to known deterministic dynamics: $x_{t+1} = f(x_t, u_t)$. Let $m^* : \mathcal{X} \rightarrow \{-1,1\}$ be a function specifying the \textit{true} occupancy of the environment by labeling states as either feasible ($-1$) or infeasible ($1$). Let $\mathcal{M}$ be the space of possible environment realizations $m^*$. Let $c^* : \mathcal{X} \times \mathcal{U} \times \mathcal{M} \rightarrow \mathbb{R}_{\ge 0}$ be a cost function specifying desirable robot behavior in a given environment, e.g., according to an expert user or an optimal design. We assume that the robot does not have access to either the true occupancy map $m^*$ or the true cost function $c^*$. However, the robot is able to make observations $z_t \in \mathcal{Z}$ of the environment in its vicinity, whose distribution depends on the robot state $x_t$ and the environment $m^*$. Suppose that a training set $\mathcal{D} := \crl{(x_{t,n},u_{t,n}^*,z_{t,n})}_{t=1, n=1}^{T_n, N}$ of $N$ expert trajectories with length $T_n$ is available to demonstrate desirable behavior. Based on the prior experience $\mathcal{D}$, our goal is to learn a cost function estimate $\hat{c}_t^{\theta} : \mathcal{X} \times \mathcal{U} \times \mathcal{Z}^t \rightarrow \mathbb{R}_{\ge 0}$, which depends on the observation sequences $z_{1:t}$ from the true latent environment and is parameterized by $\theta$. The cost function estimate can be used to specify the robot behavior in new environments. In particular, once $\hat{c}_t^\theta$ is learned, i.e., the parameters $\theta$ are fixed, the robot can execute a new navigation task by computing a control policy $\pi_t^{\theta}(\cdot|x_t)$, mapping from a state $x_t$ to a control distribution, based on $\hat{c}_t^\theta$, as follows.
\begin{problem}
\label{pb:1}
Given the cost function $\hat{c}_t^{\theta}$ at time $t$, find the optimal cost-to-go values of each control at the current robot state $x_t$,
\begin{align}
    Q^*_t(x_t, u_t) &= \hat{c}_t^\theta(x_t, u_t) \notag\\
    &+ \min_{u_{t+1:T-1}} \sum_{k=t+1}^{T-1} \hat{c}_t^\theta(x_k, u_k|z_{1:t}),\;  \forall \; u_t \in  \mathcal{U} \label{eq:pb:1}\\
    \text{s.t.} \; & x_{k+1} = f(x_k, u_k), \text{for } k = t+1, \cdots, T-1, \notag \\
            \;&  x_T = x_g. \notag 
\end{align}
\end{problem}
%Prob.~\ref{pb:1} defines the planning problem: given the parameterized cost function $\hat{c}_t^{\theta}$ whose input is $z_{1:t}$ and $\theta$, find a policy that minimizes the expected sum of costs while ensuring that the robot satisfies the state transition dynamics and reaches the goal. The planning horizon $T$ is set to be an upper bound on the number of steps in an optimal trajectory and the control space $\mathcal{U}$ is augmented to include a null control which does not change the robot state and induces zero cost once the robot reaches the goal region $\mathcal{X}_{goal}$. \\ \\

Solving Problem~\ref{pb:1} is only half the challenge. The robot also has to learn $\hat{c}_t^{\theta}$ so that the inferred policy from Problem~\ref{pb:1} obtains low cost according to the true hidden cost function $c^*$. In practice, it is not possible to query the true cost $c^*$ directly, but demonstrations (e.g., from a human navigating in an unknown environment based on visual information) can be used to indirectly optimize $\hat{c}_t^{\theta}$ as follows:
\begin{problem}
\label{pb:2}
Given demonstrations $\mathcal{D} = \crl{(x_{t,n},u_{t,n}^*,z_{t,n})}_{t=1,n=1}^{T_n, N}$, optimize the cost function parameters $\theta$ such that the cross-entropy between the policy computed in Problem~\ref{pb:1} and the demonstrated controls is minimized:
\begin{equation}
\label{eq:loss}
\begin{aligned}
    \min_{\theta} \;\;& \mathcal{L}(\theta) := \sum_{n=1}^N \sum_{t=1}^{T_n} -\log \pi_{t, n}^{\theta} (u_{t,n}^*|x_{t,n}) \\ 
    \text{s.t.} \;\;& \pi_{t,n}^{\theta}(u_{t,n}|x_{t,n}) = \frac{\exp(-Q^*_{t,n}(x_{t,n}, u_{t,n}))}{\sum_{u \in \mathcal{U}}\exp(-Q^*_{t,n}(x_{t,n}, u))}, \\
    & Q^*_{t,n}(x_{t,n}, u_{t,n}) = \text{Problem~\ref{pb:1}}(x_{t,n}, z_{1:t,n}, x_{g,n}, \theta)
\end{aligned}
\end{equation}
where $x_{g,n}$ is the goal state in each demonstration.
\end{problem}
Note that the policy that attains the minimum for $Q^*$ in Prob.\ref{pb:1} is deterministic while the robot's policy for planning in Prob.\ref{pb:2} is stochastic with bounded rationality weighted exponentially over the values of each control.

The problem setup is illustrated in Fig.~\ref{fig:approach}. While Problem~\ref{pb:1} is a standard planning problem, the challenge is to make the optimization in~\eqref{eq:pb:1} differentiable with respect to the cost function parameterization $\theta$. The latter is necessary because Problem~\ref{pb:1} appears as a nested optimization in Problem~\ref{pb:2}. This is also illustrated in Fig.~\ref{fig:approach}, where the loss has to backpropagate through the planning algorithm to update the cost parameters $\theta$.


Our approach to Problem~\ref{pb:2} is to encode a cost function representation and a planning algorithm in a differentiable computation graph, and optimize the parameters $\theta$ via gradient descent. In Sec.~\ref{sec:cost_rep}, we propose a neural network model for $\hat{c}_t^\theta$ with inputs $x \in \mathcal{X}$, $u\in\mathcal{U}$, and $z_{1:t} \in \mathcal{Z}^t$ and parameters $\theta$. In Sec.~\ref{sec:diff_plan}, we develop an efficient planning algorithm that returns a stochastic policy $\pi_t^{\theta}$ for a fixed cost function $\hat{c}_t^{\theta}$, while ensuring that $\pi_t^{\theta}$ is differentiable with respect to $\hat{c}_t^{\theta}$. Finally, in Sec.~\ref{sec:cost_learning_planning}, we combine the cost representation and the planning algorithm to optimize the performance loss $\mathcal{L}(\theta)$ of the inferred policy $\pi_t^{\theta}$ compared with the demonstrations $\mathcal{D}$ using gradient descent over the parameters $\theta$.







==> tex/old/RelatedWork.tex <==
\section{Related Work}
\label{sec:related_work}

% Traditional mapping and planning, considered as separate topics
Safe and robust autonomous navigation is difficult to achieve in unknown and unstructured environments. Traditional approaches consider mapping and planning as independent processes. A robot first maps the geometric structure of the environment from sensory data and then plans a path through the constructed map. Simultaneous localization and mapping (SLAM)~\cite{Mur_ORBSLAM15, Newcombe_KF11, Whelan_EF16, Zhang_LOAM14} has received considerable attention in the robotics community. Mature techniques utilizing various sensors, such as inertial measurement units, lidars, and RGB(D) cameras, exist. Related to this work, are techniques that focus on occupancy mapping in the context of autonomous navigation~\cite{Erdem_GoalNav12,Hornung_Octomap13,voxblox}. Given a probabilistic model of environment occupancy, there exist mature planning techniques~\cite{Kavraki_PRM94,Lavalle_RRT98,Karaman_RRTstar11,Hart_Astar68,ARA} with theoretical guarantees of finding a feasible trajectory if one exists.

%Mapping has received considerable attention in the context of simultaneous localization and mapping (SLAM)~\cite{Mur_ORBSLAM15, Newcombe_KF11, Whelan_EF16, Zhang_LOAM14}, fusing various sensorswith high-dimensional data like point clouds, RGB and RGB-D images. Occupancy grid mapping~\cite{Thrun_PR05} is widely used as a probabilistic model in robotics. In fact, grid-like decomposition of the environment is shown to be crucial for spatial navigation~\cite{Erdem_GoalNav12}. Hornung et. al. (\citeyear{Hornung_Octomap13}) further exploits the octree data structure~\cite{Samet_Octree88} for hierarchical and unbalanced environment resolution while keeping the representation probabilistic, updatable and compact. Planning algorithms in such constructed maps are studied in ~\cite{Kavraki_PRM94, Lavalle_RRT98, Karaman_RRTstar11, Hart_Astar68,ARA} with theoretical guarantees of finding a path (or in probability) between desired states.  

% Our work, among others, optimizes mapping and planning jointly
As an alternative to the traditional approach, reinforcement learning (RL) methods combine the two stages by simultaneously generating a cost function and a control policy. Recent successful techniques~\cite{Mnih_DQN15, Oh_ActPred15, Mirowski_LearnNav16, Levine_DeepVisuo16, Oh_VPN17} in deep reinforcement learning (DRL) rely on end-to-end gradient-descent optimization to directly learn a policy function from high-dimensional sensory data. Tamar et. al. (\cite{Tamar_VIN16}) introduced Value Iteration Networks (VIN), a fully differentiable neural network architecture that approximates the value iteration algorithm and can learn to plan. Inspired by VIN, Okada at el. (\cite{Okada_PIN17}) proposed path integral networks in which the control sequence resulting from the path integral control algorithm is differentiable with respect to the parameters of the controller. Our work is motivated by the same idea that automatic differentiation can be used in end-to-end optimization and we propose a differentiable A* planning algorithm to compute a control policy, while ensuring that it is differentiable with respect to the cost function parameterization. We choose to design a differentiable version of A* because of its ability to prioritize the search for an optimal trajectory using a heuristic function, thus reducing computation complexity. The prioritized search is reminiscent of the attention mechanism in visual object recognition~\cite{Cho_Attention15,Xu_Attention15,Mnih_Attention14}, where convolutional operations are not performed uniformly on an image but adaptively and sequentially on subsets of the pixels.

%However, the underlying planning algorithms are different. In this work, we use an A* planner to solve for an optimal path while ensuring the output policy is differentiable with respect to the parameters of the cost function. Gradients for improving the policy performance can be backpropagated through the planner to update the cost function parameterization. We choose the A* planning algorithm for its efficiency and scalability on large environments as it prioritize the search of an optimal path using a heuristic function. This is reminiscent of the attention mechanism in visual object recognition~\cite{Cho_Attention15, Xu_Attention15, Mnih_Attention14}, where convolutional operation is not performed uniformly on an image but adaptively and sequentially on subsets of the pixels. 

% IRL, IL, unknown noisy environment
Our work is related to the inverse reinforcement learning (IRL) problem ~\cite{Ziebart_MaxEnt08,Ng_IRL00,Hadfield_IRD17} where the goal is to infer a cost function for which the expert policy is optimal. We are interested in learning a cost function because as Ng and Russell~\cite{Ng_IRL00} argued, the cost function is a more succinct and robust description of the task. Since the problem of inferring cost from demonstration is ill-posed, e.g. the cost function that explains a set of demonstrations is not unique, several works have made theoretical assumptions on the form of policy to be solved. For example, beyond matching the expert's behavior, ~\cite{Ratliff_06} looks for a policy that has maximum margin with others and ~\cite{Ziebart_MaxEnt08} assumes expert suboptimality and solves for one that has maximum entropy. Other approaches relevant to our work are those that consider planning in unknown environments with partial and noisy observations. \TW{add more reference here from the reviewers' comments}

% Partially observed environments, memory ...
Recent works~\cite{Khan_MACN18,Gupta_CMP17,Heess_Memory15} leverage neural network memory architectures to process partial observations, store spatial regularities and, in turn, generate a reactive control policy. While these works propose methods for joint optimization of a latent map representation and inferring control policies, our contribution is in bringing the well-known A* search algorithm in the end-to-end differentiable architecture. 



%Traditional motion planning algorithms like A*~\cite{ARA} look for complete solutions in a discretization of the continuous state space. A* takes advantage of a heuristic function to guide the search for an optimal path on a graph or a discretization of the continuous state space. However, a small change in the environment might result in an infeasible path and A* would consider it as a new problem instance and solve it from scratch, making it inefficient for real-world deployments. Extensions of A*~\cite{LPA,D} fix the problem by considering incremental solutions when the environment is partially unknown or changing. For example, D* updates the edge costs in a path to the goal when new space configuration is observed. It then recomputes the current position to goal while reusing as much information as possible. Our work is similar as we are also considering incremental solutions in a partially unknown environment. However, we emphasize that in our work, the latent map representation and the induced edge cost are incrementally optimized by learning which features are important through solving the navigation task. The latent map not only captures which obstacles are observed versus which are not, but also learns which are important and which are trivial. \\ \\
%Planning algorithms in the reinforcement learning aim at finding an optimal policy by utilizing an available or learned dynamics model. Tamar et al.~\cite{VIN_NIPS16} introduced value iteration networks (VIN), a fully differentiable neural network architecture that can learn to plan. It embeds a planning module that approximates the value iteration algorithm through a series of convolutional and maxpooling layers. The neural network architecture learns a reward map and transition dynamics of the environment, applies approximate value iteration algorithm and returns a reactive policy. The Dyna algorithm~\cite{SuttonRL} naturally interleaves learning and planning. Learning with real experience and planning with simulated experience are regarded as similar approaches since they are both methods to improve the estimated value functions with backup operations. Learning and planning are parallel threads in the Dyna architecture and they can process as fast as the computation resource allows without waiting for each other to take turns. In ~\cite{Predictron,VPN,ATreeC}, the differentiable dynamics model is learned to generate multi-step rollouts of simulated experience in order to get an accurate approximation of the value function. Our work assumes known dynamics and we are only interested in learning what is a good representation of the cost that achieves well in navigation tasks. \\ \\
%Okada at el.~\cite{PIN} proposed path integral networks (PIN) that focuses on the path integral optimal control algorithm for model predictive control. PIN is inspired conceptually by VIN to look for a planning algorithm that is differentiable end-to-end. Their observation is that the control sequence resulting from the path integral control algorithm are differentiable with respect to all of the controller internal parameters. Our work is motivated by the same idea that we could use the standard deep learning tools like backpropagation and automatic differentiation for optimization. However, the underlying algorithms are different. In this work, we use an A* planner to solve for an optimal path on a graph, while ensuring that the planner output policy is differentiable with respect to the parameters of the latent map. Gradients on improving the policy performance can be backpropagated through the planner to update the latent map representation. \\ \\
%Our work is also related to the attention mechanism in visual object recognition~\cite{Cho15, Xu15, Attention}. Mnih et al.~\cite{Attention} used a recurrent neural network that solves image recognition task by processing different resolutions of selected regions in a image. This is more computationally efficient than applying a convolutional layer on the entire image. Our work is inspired by the attention mechanism that we do need to apply dynamic programming over the entire state space, as is done in VIN. Rather, we can use an A* planner to prioritize the search of promising states with the guide of a heuristic function. \\ \\
%Prior works~\cite{Ha18, Kurutach18} used variational autoencoder~\cite{Blei16, Goodfellow-et-al-2016} and generative adversarial networks~\cite{GAN14} to learn plannable latent representations in domains with high-dimensional observations. However, these works focus on learning the representation and dynamics model in an end-to-end fashion so that the policy maximizes the expected sum of rewards in the reinforcement learning setting~\cite{Srinivas18, Oh15, Finn16}. In our work, we assume a deterministic and known dynamics model and we learn a latent map representation only to infer a cost function that enables efficient search of a feasible path. \\ \\
%Inverse reinforcement learning~\cite{Ziebart08, Ng_Russell00} problem optimizes a cost function from demonstrations of an approximately optimal policy. Our problem is similar as both are inferring an unobserved cost function, but we do not have the maximum entropy assumption of the optimality behavior of the expert~\cite{Ziebart08}. In this sense, our problem is also related to imitation learning~\cite{GAIL16} in which the problem is to learn a policy by mimicking an expert policy. However, we explicitly design a parameterized cost function that can learn from and can be used by a planning algorithm.\NA{This is a general comment for the whole Intro section. You should shorten it a bit and also conclude with a bulleted list of our contributions. The main things to emphasize are something along the lines of: 1) we learn a latent environment representation from partial observations, 2) we propose a differentiable planning algorithm that performs only local convolution operations encoding Bellman backups on a subset of promising states, 3) our algorithm allows learning an implicit environment representation and an associated task-specific cost function from expert demonstrations by differentiating through both the planning and cost representation stages...}

